Evaluating Explanation Methods for Deep Learning in Security

Deep learning is increasingly used as a building block of security systems. Unfortunately, neural networks are hard to interpret and typically opaque to the practitioner. The machine learning community has started to address this problem by developing methods for explaining the predictions of neural networks. While several of these approaches have been successfully applied in the area of computer vision, their application in security has received little attention so far. It is an open question which explanation methods are appropriate for computer security and what requirements they need to satisfy. In this paper, we introduce criteria for comparing and evaluating explanation methods in the context of computer security. These cover general properties, such as the accuracy of explanations, as well as security-focused aspects, such as the completeness, efficiency, and robustness. Based on our criteria, we investigate six popular explanation methods and assess their utility in security systems for malware detection and vulnerability discovery. We observe significant differences between the methods and build on these to derive general recommendations for selecting and applying explanation methods in computer security.

==> tables/153126-color.c-lemna.tex <==
\begin{codelst}
(*@\hlc[pro!67]{VAR0}@*) (*@\hlc[pro!62]{=}@*) (*@\hlc[pro!60]{FUN0}@*) (*@\hlc[pro!58]{(}@*) (*@\hlc[pro!56]{VAR1}@*) (*@\hlc[pro!54]{[}@*) (*@\hlc[pro!53]{VAR2}@*) (*@\hlc[pro!52]{]}@*) (*@\hlc[pro!51]{,}@*) (*@\hlc[pro!51]{STR0}@*) (*@\hlc[pro!50]{,}@*) (*@\hlc[pro!49]{\&}@*) (*@\hlc[pro!49]{VAR3}@*) (*@\hlc[pro!49]{)}@*) (*@\hlc[pro!49]{;}@*)
(*@\hlc[pro!49]{VAR0}@*) (*@\hlc[pro!50]{=}@*) (*@\hlc[pro!52]{strcpy}@*) (*@\hlc[pro!96]{(}@*) (*@\hlc[pro!98]{(}@*) (*@\hlc[pro!99]{FUN0}@*) (*@\hlc[pro!100]{(}@*) (*@\hlc[pro!100]{strlen}@*) (*@\hlc[pro!100]{(}@*) (*@\hlc[pro!99]{VAR1}@*) (*@\hlc[pro!87]{[}@*) (*@\hlc[pro!86]{INT0}@*) (*@\hlc[pro!84]{]}@*) (*@\hlc[pro!83]{)}@*) (*@\hlc[pro!82]{+}@*) (*@\hlc[pro!81]{INT0}@*) (*@\hlc[pro!80]{)}@*) (*@\hlc[pro!79]{)}@*) (*@\hlc[pro!78]{,}@*) (*@\hlc[pro!77]{VAR1}@*) (*@\hlc[pro!75]{[}@*) (*@\hlc[pro!74]{INT0}@*) (*@\hlc[pro!54]{]}@*) (*@\hlc[pro!53]{)}@*) (*@\hlc[pro!52]{;}@*)
\end{codelst}

==> tables/153126-color.c-lrp.tex <==
\begin{codelst}
(*@\hlc[pro!18]{VAR0}@*) (*@\hlc[pro!30]{=}@*) (*@\hlc[pro!3]{FUN0}@*) (*@\hlc[pro!3]{(}@*) (*@\hlc[pro!6]{VAR1}@*) (*@\hlc[con!14]{[}@*) (*@\hlc[pro!16]{VAR2}@*) (*@\hlc[con!45]{]}@*) (*@\hlc[con!18]{,}@*) (*@\hlc[pro!100]{STR0}@*) (*@\hlc[con!44]{,}@*) (*@\hlc[con!13]{\&}@*) (*@\hlc[pro!15]{VAR3}@*) (*@\hlc[pro!1]{)}@*) (*@\hlc[con!12]{;}@*)
(*@\hlc[pro!12]{VAR0}@*) (*@\hlc[con!6]{=}@*) (*@\hlc[con!89]{strcpy}@*) (*@\hlc[pro!18]{(}@*) (*@\hlc[pro!13]{(}@*) (*@\hlc[con!16]{FUN0}@*) (*@\hlc[pro!16]{(}@*) (*@\hlc[pro!38]{strlen}@*) (*@\hlc[pro!6]{(}@*) (*@\hlc[con!0]{VAR1}@*) (*@\hlc[con!12]{[}@*) (*@\hlc[pro!34]{INT0}@*) (*@\hlc[con!21]{]}@*) (*@\hlc[pro!14]{)}@*) (*@\hlc[pro!31]{+}@*) (*@\hlc[pro!1]{INT0}@*) (*@\hlc[pro!1]{)}@*) (*@\hlc[pro!0]{)}@*) (*@\hlc[con!1]{,}@*) (*@\hlc[con!0]{VAR1}@*) (*@\hlc[pro!0]{[}@*) (*@\hlc[pro!1]{INT0}@*) (*@\hlc[con!0]{]}@*) (*@\hlc[pro!0]{)}@*) (*@\hlc[con!2]{;}@*)
\end{codelst}

==> tables/68403-CWE122-Heap-Based-Buffer-Overflow--cpp-CWE805-char-memmove-22.cpp-lemna.tex <==
\begin{codelst}
(*@\hlc[pro!100]{char}@*) (*@\hlc[pro!100]{*}@*) (*@\hlc[pro!99]{VAR0}@*) (*@\hlc[pro!98]{;}@*)
(*@\hlc[pro!98]{VAR0}@*) (*@\hlc[pro!97]{=}@*) (*@\hlc[pro!96]{NULL}@*) (*@\hlc[pro!41]{;}@*)
(*@\hlc[pro!41]{VAR0}@*) (*@\hlc[pro!41]{=}@*) (*@\hlc[pro!45]{INT0}@*) (*@\hlc[pro!47]{;}@*)
(*@\hlc[pro!57]{VAR0}@*) (*@\hlc[pro!57]{=}@*) (*@\hlc[pro!58]{FUN0}@*) (*@\hlc[pro!57]{(}@*) (*@\hlc[pro!57]{VAR0}@*) (*@\hlc[pro!50]{)}@*) (*@\hlc[pro!40]{;}@*)
(*@\hlc[pro!38]{char}@*) (*@\hlc[pro!36]{*}@*) (*@\hlc[pro!35]{FUN0}@*) (*@\hlc[pro!33]{(}@*) (*@\hlc[pro!31]{char}@*) (*@\hlc[pro!29]{*}@*) (*@\hlc[pro!28]{VAR0}@*) (*@\hlc[pro!26]{)}@*)
(*@\hlc[pro!26]{if}@*) (*@\hlc[pro!25]{(}@*) (*@\hlc[pro!25]{VAR0}@*) (*@\hlc[pro!26]{)}@*)
(*@\hlc[pro!27]{VAR0}@*) (*@\hlc[pro!28]{=}@*) (*@\hlc[pro!29]{new}@*) (*@\hlc[pro!32]{char}@*) (*@\hlc[pro!33]{[}@*) (*@\hlc[pro!34]{INT0}@*) (*@\hlc[pro!35]{]}@*) (*@\hlc[pro!35]{;}@*)
(*@\hlc[pro!36]{VAR0}@*) (*@\hlc[pro!37]{[}@*) (*@\hlc[pro!39]{INT0}@*) (*@\hlc[pro!40]{]}@*) (*@\hlc[pro!41]{=}@*) (*@\hlc[pro!43]{STR0}@*) (*@\hlc[pro!48]{;}@*)
(*@\hlc[pro!50]{return}@*) (*@\hlc[pro!51]{VAR0}@*) (*@\hlc[pro!52]{;}@*)
(*@\hlc[pro!52]{char}@*)
\end{codelst}

==> tables/68403-CWE122-Heap-Based-Buffer-Overflow--cpp-CWE805-char-memmove-22.cpp-lrp.tex <==
\begin{codelst}
(*@\hlc[pro!1]{char}@*) (*@\hlc[pro!5]{*}@*) (*@\hlc[con!39]{VAR0}@*) (*@\hlc[con!8]{;}@*)
(*@\hlc[pro!18]{VAR0}@*) (*@\hlc[pro!100]{=}@*) (*@\hlc[con!3]{NULL}@*) (*@\hlc[con!51]{;}@*)
(*@\hlc[pro!7]{VAR0}@*) (*@\hlc[con!3]{=}@*) (*@\hlc[con!3]{INT0}@*) (*@\hlc[pro!6]{;}@*)
(*@\hlc[con!4]{VAR0}@*) (*@\hlc[con!17]{=}@*) (*@\hlc[con!3]{FUN0}@*) (*@\hlc[con!0]{(}@*) (*@\hlc[pro!4]{VAR0}@*) (*@\hlc[con!5]{)}@*) (*@\hlc[pro!5]{;}@*)
(*@\hlc[pro!4]{char}@*) (*@\hlc[pro!18]{*}@*) (*@\hlc[pro!1]{FUN0}@*) (*@\hlc[pro!8]{(}@*) (*@\hlc[pro!13]{char}@*) (*@\hlc[con!10]{*}@*) (*@\hlc[con!10]{VAR0}@*) (*@\hlc[con!3]{)}@*)
(*@\hlc[con!1]{if}@*) (*@\hlc[pro!4]{(}@*) (*@\hlc[pro!9]{VAR0}@*) (*@\hlc[pro!7]{)}@*)
(*@\hlc[con!4]{VAR0}@*) (*@\hlc[con!3]{=}@*) (*@\hlc[pro!13]{new}@*) (*@\hlc[pro!60]{char}@*) (*@\hlc[con!14]{[}@*) (*@\hlc[con!26]{INT0}@*) (*@\hlc[pro!2]{]}@*) (*@\hlc[con!13]{;}@*)
(*@\hlc[con!2]{VAR0}@*) (*@\hlc[con!12]{[}@*) (*@\hlc[con!2]{INT0}@*) (*@\hlc[con!24]{]}@*) (*@\hlc[con!6]{=}@*) (*@\hlc[con!1]{STR0}@*) (*@\hlc[pro!1]{;}@*)
(*@\hlc[con!6]{return}@*) (*@\hlc[pro!2]{VAR0}@*) (*@\hlc[pro!2]{;}@*)
(*@\hlc[pro!1]{char}@*)
\end{codelst}

==> tables/78503-CWE127-Buffer-Underread--new-wchar-t-cpy-82-bad.cpp-lemna.tex <==
\begin{codelst}
(*@\hlc[con!30]{wchar\_t}@*) (*@\hlc[con!29]{*}@*) (*@\hlc[con!28]{VAR0}@*) (*@\hlc[con!27]{;}@*)
(*@\hlc[con!25]{VAR0}@*) (*@\hlc[con!23]{=}@*) (*@\hlc[con!21]{NULL}@*) (*@\hlc[con!19]{;}@*)
(*@\hlc[con!17]{wchar\_t}@*) (*@\hlc[con!15]{*}@*) (*@\hlc[con!13]{VAR0}@*) (*@\hlc[con!12]{=}@*) (*@\hlc[con!10]{new}@*) (*@\hlc[pro!22]{wchar\_t}@*) (*@\hlc[pro!23]{[}@*) (*@\hlc[pro!25]{INT0}@*) (*@\hlc[pro!27]{]}@*) (*@\hlc[pro!28]{;}@*)
(*@\hlc[pro!30]{wmemset}@*) (*@\hlc[pro!32]{(}@*) (*@\hlc[pro!34]{VAR0}@*) (*@\hlc[pro!35]{,}@*) (*@\hlc[pro!37]{STR0}@*) (*@\hlc[pro!44]{,}@*) (*@\hlc[pro!45]{INT0}@*) (*@\hlc[pro!47]{-}@*) (*@\hlc[pro!49]{INT1}@*) (*@\hlc[pro!51]{)}@*) (*@\hlc[pro!53]{;}@*)
(*@\hlc[pro!55]{VAR0}@*) (*@\hlc[pro!57]{[}@*) (*@\hlc[pro!59]{INT0}@*) (*@\hlc[pro!61]{-}@*) (*@\hlc[pro!100]{INT1}@*) (*@\hlc[pro!100]{]}@*) (*@\hlc[pro!99]{=}@*) (*@\hlc[pro!98]{STR0}@*) (*@\hlc[pro!97]{;}@*)
(*@\hlc[pro!95]{VAR0}@*) (*@\hlc[pro!94]{=}@*) (*@\hlc[pro!92]{VAR1}@*) (*@\hlc[pro!91]{-}@*) (*@\hlc[pro!90]{INT0}@*) (*@\hlc[pro!89]{;}@*)
(*@\hlc[pro!88]{VAR0}@*) (*@\hlc[pro!87]{*}@*) (*@\hlc[pro!87]{VAR1}@*) (*@\hlc[pro!86]{=}@*) (*@\hlc[pro!86]{new}@*) (*@\hlc[pro!86]{VAR2}@*)
\end{codelst}

==> tables/78503-CWE127-Buffer-Underread--new-wchar-t-cpy-82-bad.cpp-lrp.tex <==
\begin{codelst}
(*@\hlc[pro!36]{wchar\_t}@*) (*@\hlc[pro!5]{*}@*) (*@\hlc[con!13]{VAR0}@*) (*@\hlc[pro!10]{;}@*)
(*@\hlc[pro!17]{VAR0}@*) (*@\hlc[pro!35]{=}@*) (*@\hlc[pro!16]{NULL}@*) (*@\hlc[pro!0]{;}@*)
(*@\hlc[pro!16]{wchar\_t}@*) (*@\hlc[con!6]{*}@*) (*@\hlc[con!28]{VAR0}@*) (*@\hlc[con!90]{=}@*) (*@\hlc[pro!95]{new}@*) (*@\hlc[con!100]{wchar\_t}@*) (*@\hlc[con!72]{[}@*) (*@\hlc[con!13]{INT0}@*) (*@\hlc[pro!4]{]}@*) (*@\hlc[pro!14]{;}@*)
(*@\hlc[con!14]{wmemset}@*) (*@\hlc[con!4]{(}@*) (*@\hlc[pro!30]{VAR0}@*) (*@\hlc[con!8]{,}@*) (*@\hlc[pro!82]{STR0}@*) (*@\hlc[pro!56]{,}@*) (*@\hlc[con!78]{INT0}@*) (*@\hlc[pro!6]{-}@*) (*@\hlc[con!7]{INT1}@*) (*@\hlc[pro!10]{)}@*) (*@\hlc[con!5]{;}@*)
(*@\hlc[pro!2]{VAR0}@*) (*@\hlc[con!3]{[}@*) (*@\hlc[pro!19]{INT0}@*) (*@\hlc[pro!5]{-}@*) (*@\hlc[pro!3]{INT1}@*) (*@\hlc[pro!3]{]}@*) (*@\hlc[con!7]{=}@*) (*@\hlc[con!1]{STR0}@*) (*@\hlc[con!3]{;}@*)
(*@\hlc[pro!2]{VAR0}@*) (*@\hlc[con!1]{=}@*) (*@\hlc[pro!0]{VAR1}@*) (*@\hlc[pro!0]{-}@*) (*@\hlc[pro!0]{INT0}@*) (*@\hlc[pro!1]{;}@*)
(*@\hlc[con!1]{VAR0}@*) (*@\hlc[con!0]{*}@*) (*@\hlc[con!1]{VAR1}@*) (*@\hlc[pro!0]{=}@*) (*@\hlc[con!1]{new}@*) (*@\hlc[pro!0]{VAR2}@*)
\end{codelst}

==> tables/DAMD-0.tex <==
\begin{tabular}{
  cll
}
  \toprule
  \bfseries Id & \bfseries LRP & \bfseries Lemna\\
  \midrule
  0 & \cellcolor{con!1}  1. invoke-direct & \cellcolor{pro!100}  1. invoke-direct \\
  1 & \cellcolor{pro!3}  2. return-void & \cellcolor{pro!100}  2. return-void \\
  2 & \cellcolor{pro!2}  3. invoke-direct & \cellcolor{pro!100}  3. invoke-direct \\
  3 & \cellcolor{pro!19}  4. return-void & \cellcolor{pro!100}  4. return-void \\
  4 & \cellcolor{pro!25}  5. invoke-direct & \cellcolor{pro!100}  5. invoke-direct \\
  5 & \cellcolor{pro!14}  6. return-void & \cellcolor{pro!100}  6. return-void \\
  6 & \cellcolor{pro!14}  7. invoke-direct & \cellcolor{pro!100}  7. invoke-direct \\
  7 & \cellcolor{pro!45}  8. return-void & \cellcolor{pro!100}  8. return-void \\
  8 & \cellcolor{pro!48}  9. invoke-direct & \cellcolor{pro!100}  9. invoke-direct \\
  9 & \cellcolor{pro!27} 10. return-void & \cellcolor{pro!100} 10. return-void \\
  10 & \cellcolor{pro!100} 11. invoke-super & \cellcolor{pro!100} 11. invoke-super \\
  11 & \cellcolor{pro!15} 12. new-instance & \cellcolor{pro!100} 12. new-instance \\
  12 & \cellcolor{pro!38} 13. invoke-direct & \cellcolor{pro!100} 13. invoke-direct \\
  13 & \cellcolor{pro!14} 14. const-string & \cellcolor{pro!99} 14. const-string \\
  14 & \cellcolor{pro!9} 15. invoke-virtual & \cellcolor{pro!99} 15. invoke-virtual \\
  15 & \cellcolor{pro!14} 16. invoke-virtual & \cellcolor{pro!99} 16. invoke-virtual \\
  16 & \cellcolor{pro!7} 17. return-void & \cellcolor{pro!99} 17. return-void \\
  17 & \cellcolor{pro!0} 18. invoke-direct & \cellcolor{pro!99} 18. invoke-direct \\
  18 & \cellcolor{pro!9} 19. return-void & \cellcolor{pro!99} 19. return-void \\
  \bottomrule
\end{tabular}

==> tables/DAMD-1.tex <==
\begin{tabular}{
  cll
}
  \toprule
  \bfseries Id & \bfseries LRP & \bfseries Lemna\\
  \midrule
  0 & \cellcolor{con!1} invoke-direct & \cellcolor{pro!100} invoke-direct \\
  1 & \cellcolor{pro!3} return-void & \cellcolor{pro!100} return-void \\
  2 & \cellcolor{pro!2} invoke-direct & \cellcolor{pro!100} invoke-direct \\
  3 & \cellcolor{pro!19} return-void & \cellcolor{pro!100} return-void \\
  4 & \cellcolor{pro!25} invoke-direct & \cellcolor{pro!100} invoke-direct \\
  5 & \cellcolor{pro!14} return-void & \cellcolor{pro!100} return-void \\
  6 & \cellcolor{pro!14} invoke-direct & \cellcolor{pro!100} invoke-direct \\
  7 & \cellcolor{pro!45} return-void & \cellcolor{pro!100} return-void \\
  8 & \cellcolor{pro!48} invoke-direct & \cellcolor{pro!100} invoke-direct \\
  9 & \cellcolor{pro!27} return-void & \cellcolor{pro!100} return-void \\
  10 & \cellcolor{pro!100} invoke-super & \cellcolor{pro!100} invoke-super \\
  11 & \cellcolor{pro!15} new-instance & \cellcolor{pro!100} new-instance \\
  12 & \cellcolor{pro!38} invoke-direct & \cellcolor{pro!100} invoke-direct \\
  13 & \cellcolor{pro!14} const-string & \cellcolor{pro!99} const-string \\
  14 & \cellcolor{pro!9} invoke-virtual & \cellcolor{pro!99} invoke-virtual \\
  15 & \cellcolor{pro!14} invoke-virtual & \cellcolor{pro!99} invoke-virtual \\
  16 & \cellcolor{pro!7} return-void & \cellcolor{pro!99} return-void \\
  17 & \cellcolor{pro!0} invoke-direct & \cellcolor{pro!99} invoke-direct \\
  18 & \cellcolor{pro!9} return-void & \cellcolor{pro!99} return-void \\
  \bottomrule
\end{tabular}

==> tables/Mimicus-0.tex <==
\begin{tabular}{
  cll
}
  \toprule
  \bfseries Id & \bfseries lrp & \bfseries lemna\\
  \midrule
  0 & \cellcolor{green!100} count\_javascript & \cellcolor{green!100} count\_javascript \\
  1 & \cellcolor{green!75.99179000000001} count\_js & \cellcolor{green!82.09895252879011} count\_js \\
  2 & \cellcolor{green!15.848137000000001} count\_trailer & \cellcolor{green!68.83739214883579} count\_trailer \\
  3 & \cellcolor{green!13.460113000000002} count\_endobj & \cellcolor{green!20.816360267660396} count\_endobj \\
  4 & \cellcolor{green!11.0375} createdate\_tz & \cellcolor{green!29.7690837508515} createdate\_tz \\
  5 & \cellcolor{green!10.085318000000001} count\_box\_letter & \cellcolor{green!58.91945765423573} count\_box\_letter \\
  6 & \cellcolor{green!9.6530065} pos\_page\_avg & \cellcolor{green!59.886716309771174} pos\_page\_avg \\
  7 & \cellcolor{green!9.098243} pos\_page\_min & \cellcolor{green!45.31511431240563} pos\_page\_min \\
  8 & \cellcolor{green!8.137962} count\_stream & \cellcolor{green!9.186005424822106} count\_stream \\
  9 & \cellcolor{green!8.059467} ratio\_size\_stream & \cellcolor{red!3.3466406192237397} ratio\_size\_stream \\
  10 & \cellcolor{green!6.568932500000001} pos\_page\_max & \cellcolor{red!26.168092873203967} pos\_page\_max \\
  11 & \cellcolor{green!6.366721} len\_obj\_min & \cellcolor{green!34.415249095674014} len\_obj\_min \\
  12 & \cellcolor{green!6.302773} count\_page & \cellcolor{green!21.1763803879927} count\_page \\
  13 & \cellcolor{green!5.5483066} moddate\_ts & \cellcolor{green!69.45506439940378} moddate\_ts \\
  14 & \cellcolor{green!4.672780299999999} pos\_box\_avg & \cellcolor{green!27.404251302853705} pos\_box\_avg \\
  15 & \cellcolor{green!3.9392304000000005} pos\_acroform\_avg & \cellcolor{green!0.14010753226153105} pos\_acroform\_avg \\
  16 & \cellcolor{green!3.5963714} createdate\_ts & \cellcolor{red!7.346178172196789} createdate\_ts \\
  17 & \cellcolor{green!3.5722703} box\_nonother\_types & \cellcolor{green!7.258526749976101} box\_nonother\_types \\
  18 & \cellcolor{green!3.1876538} len\_obj\_max & \cellcolor{green!36.9990058466322} len\_obj\_max \\
  19 & \cellcolor{green!3.1770411999999997} pos\_acroform\_min & \cellcolor{green!44.77186906411376} pos\_acroform\_min \\
  20 & \cellcolor{green!3.148493} pos\_box\_min & \cellcolor{green!22.450217450419313} pos\_box\_min \\
  21 & \cellcolor{green!2.1687713} ratio\_size\_page & \cellcolor{red!14.075640993390149} ratio\_size\_page \\
  22 & \cellcolor{green!2.0982893} pos\_image\_avg & \cellcolor{green!3.616443496116343} pos\_image\_avg \\
  23 & \cellcolor{green!1.9331591} pos\_acroform\_max & \cellcolor{green!28.733736869346018} pos\_acroform\_max \\
  24 & \cellcolor{green!1.6792000000000002} len\_stream\_min & \cellcolor{red!31.789710122669273} len\_stream\_min \\
  25 & \cellcolor{green!0.8499469000000001} pos\_image\_max & \cellcolor{green!21.913493552166788} pos\_image\_max \\
  26 & \cellcolor{green!0.20840566000000002} pos\_box\_max & \cellcolor{green!34.37779868851627} pos\_box\_max \\
  27 & \cellcolor{red!0.013970964999999998} count\_obj & \cellcolor{red!45.553025937522264} count\_obj \\
  28 & \cellcolor{red!0.09056418000000001} createdate\_version\_ratio & \cellcolor{green!7.360348407160043} createdate\_version\_ratio \\
  29 & \cellcolor{red!0.4695176} len\_obj\_avg & \cellcolor{red!1.5666128612895138} len\_obj\_avg \\
  30 & \cellcolor{red!0.6162671} count\_action & \cellcolor{green!58.982200730077594} count\_action \\
  31 & \cellcolor{red!1.2671540000000001} pos\_image\_min & \cellcolor{red!8.399280786494872} pos\_image\_min \\
  32 & \cellcolor{red!1.4000183} version & \cellcolor{green!16.136483386151134} version \\
  33 & \cellcolor{red!1.8416094} count\_startxref & \cellcolor{red!7.16493404385876} count\_startxref \\
  34 & \cellcolor{red!2.1882787} ratio\_size\_obj & \cellcolor{green!30.934556462360607} ratio\_size\_obj \\
  35 & \cellcolor{red!2.2008736} len\_stream\_avg & \cellcolor{green!4.85457770672548} len\_stream\_avg \\
  36 & \cellcolor{red!3.292667} moddate\_tz & \cellcolor{red!23.70977475640401} moddate\_tz \\
  37 & \cellcolor{red!5.007391} pos\_eof\_max & \cellcolor{red!31.61558685535118} pos\_eof\_max \\
  38 & \cellcolor{red!5.3490248} size & \cellcolor{red!34.138504342782674} size \\
  39 & \cellcolor{red!5.9607826} moddate\_version\_ratio & \cellcolor{red!23.351211788396874} moddate\_version\_ratio \\
  40 & \cellcolor{red!7.874717} count\_endstream & \cellcolor{red!8.382242734728006} count\_endstream \\
  41 & \cellcolor{red!9.080968} pos\_eof\_avg & \cellcolor{red!1.2323799375947766} pos\_eof\_avg \\
  42 & \cellcolor{red!10.111334} count\_xref & \cellcolor{green!3.099369070762764} count\_xref \\
  43 & \cellcolor{red!13.336954} count\_eof & \cellcolor{green!6.309838716474489} count\_eof \\
  44 & \cellcolor{red!15.077621999999998} count\_box\_other & \cellcolor{red!42.834293511763065} count\_box\_other \\
  45 & \cellcolor{red!17.627679} pos\_eof\_min & \cellcolor{red!9.852799417167896} pos\_eof\_min \\
  46 & \cellcolor{red!17.801605000000002} len\_stream\_max & \cellcolor{red!34.21267019198955} len\_stream\_max \\
  \bottomrule
\end{tabular}

==> tables/My-Freaky-APK.tex <==
\begin{tabular}{
  clll
}
  \toprule
  \bfseries Id & \bfseries LRP & \bfseries LEMNA & \bfseries LinReg\\
  \midrule
  0 & \cellcolor{pro!100} feature::android.hardware.touchscreen & \cellcolor{pro!0} feature::android.hardware.touchscreen & \cellcolor{pro!100} feature::android.hardware.touchscreen \\
  1 & \cellcolor{pro!57} intent::android.intent.category.LAUNCHER & \cellcolor{pro!0} intent::android.intent.category.LAUNCHER & \cellcolor{pro!48} intent::android.intent.category.LAUNCHER \\
  2 & \cellcolor{pro!35} real\_permission::android.permission.ACCESS\_WIFI\_STATE & \cellcolor{pro!0} real\_permission::android.permission.ACCESS\_WIFI\_STATE & \cellcolor{pro!26} real\_permission::android.permission.ACCESS\_WIFI\_STATE \\
  3 & \cellcolor{pro!30} intent::android.intent.action.VIEW & \cellcolor{pro!0} intent::android.intent.action.VIEW & \cellcolor{pro!70} intent::android.intent.action.VIEW \\
  4 & \cellcolor{pro!26} url::schemas.android.com & \cellcolor{pro!0} url::schemas.android.com & \cellcolor{pro!48} url::schemas.android.com \\
  5 & \cellcolor{pro!26} intent::android.intent.category.DEFAULT & \cellcolor{pro!0} intent::android.intent.category.DEFAULT & \cellcolor{pro!72} intent::android.intent.category.DEFAULT \\
  6 & \cellcolor{pro!26} real\_permission::android.permission.INTERNET & \cellcolor{pro!0} real\_permission::android.permission.INTERNET & \cellcolor{pro!66} real\_permission::android.permission.INTERNET \\
  7 & \cellcolor{pro!23} api\_call::android/webkit/WebView & \cellcolor{pro!0} api\_call::android/webkit/WebView & \cellcolor{pro!0} api\_call::android/webkit/WebView \\
  8 & \cellcolor{pro!18} url::a.admob.com & \cellcolor{pro!0} url::a.admob.com & \cellcolor{pro!2} url::a.admob.com \\
  9 & \cellcolor{pro!18} feature::android.hardware.screen.portrait & \cellcolor{pro!0} feature::android.hardware.screen.portrait & \cellcolor{pro!18} feature::android.hardware.screen.portrait \\
  10 & \cellcolor{pro!17} url::http://a.admob.com/f0? & \cellcolor{pro!0} url::http://a.admob.com/f0? & \cellcolor{pro!49} url::http://a.admob.com/f0? \\
  11 & \cellcolor{pro!15} call::getSystemService & \cellcolor{pro!0} call::getSystemService & \cellcolor{pro!0} call::getSystemService \\
  12 & \cellcolor{pro!11} call::getPackageInfo & \cellcolor{pro!0} call::getPackageInfo & \cellcolor{pro!0} call::getPackageInfo \\
  13 & \cellcolor{pro!8} real\_permission::android.permission.READ\_PHONE\_STATE & \cellcolor{pro!0} real\_permission::android.permission.READ\_PHONE\_STATE & \cellcolor{pro!0} real\_permission::android.permission.READ\_PHONE\_STATE \\
  14 & \cellcolor{pro!8} service\_receiver::com.google.ads.InstallReceiver & \cellcolor{pro!0} service\_receiver::com.google.ads.InstallReceiver & \cellcolor{pro!0} service\_receiver::com.google.ads.InstallReceiver \\
  15 & \cellcolor{pro!7} intent::android.intent.action.MAIN & \cellcolor{pro!0} intent::android.intent.action.MAIN & \cellcolor{pro!0} intent::android.intent.action.MAIN \\
  16 & \cellcolor{pro!5} url::https://ngpipes.ngmoco.com/pipes/r.2/bulk\_record\_stats & \cellcolor{pro!0} url::https://ngpipes.ngmoco.com/pipes/r.2/bulk\_record\_stats & \cellcolor{pro!0} url::https://ngpipes.ngmoco.com/pipes/r.2/bulk\_record\_stats \\
  17 & \cellcolor{pro!4} service\_receiver::com.ngmoco.marketingapp.NGPipesService & \cellcolor{pro!0} service\_receiver::com.ngmoco.marketingapp.NGPipesService & \cellcolor{pro!0} service\_receiver::com.ngmoco.marketingapp.NGPipesService \\
  18 & \cellcolor{pro!4} call::HttpPost & \cellcolor{pro!0} call::HttpPost & \cellcolor{pro!0} call::HttpPost \\
  19 & \cellcolor{pro!4} service\_receiver::com.ngmoco.marketservice.PlayService & \cellcolor{pro!0} service\_receiver::com.ngmoco.marketservice.PlayService & \cellcolor{pro!0} service\_receiver::com.ngmoco.marketservice.PlayService \\
  20 & \cellcolor{pro!4} url::ngpipes.ngmoco.com & \cellcolor{pro!0} url::ngpipes.ngmoco.com & \cellcolor{pro!0} url::ngpipes.ngmoco.com \\
  21 & \cellcolor{pro!4} permission::android.permission.INTERNET & \cellcolor{pro!0} permission::android.permission.INTERNET & \cellcolor{pro!0} permission::android.permission.INTERNET \\
  22 & \cellcolor{pro!3} service\_receiver::com.ngmoco.marketingapp.PackageService & \cellcolor{pro!0} service\_receiver::com.ngmoco.marketingapp.PackageService & \cellcolor{pro!0} service\_receiver::com.ngmoco.marketingapp.PackageService \\
  23 & \cellcolor{pro!3} real\_permission::android.permission.ACCESS\_NETWORK\_STATE & \cellcolor{pro!0} real\_permission::android.permission.ACCESS\_NETWORK\_STATE & \cellcolor{pro!0} real\_permission::android.permission.ACCESS\_NETWORK\_STATE \\
  24 & \cellcolor{pro!2} activity::.PackageApplication & \cellcolor{pro!0} activity::.PackageApplication & \cellcolor{pro!0} activity::.PackageApplication \\
  25 & \cellcolor{pro!2} call::Read/Write External Storage & \cellcolor{pro!0} call::Read/Write External Storage & \cellcolor{pro!0} call::Read/Write External Storage \\
  26 & \cellcolor{con!2} url::http://schemas.android.com/apk/lib/com.google.ads & \cellcolor{pro!0} url::http://schemas.android.com/apk/lib/com.google.ads & \cellcolor{pro!0} url::http://schemas.android.com/apk/lib/com.google.ads \\
  27 & \cellcolor{con!5} permission::android.permission.READ\_PHONE\_STATE & \cellcolor{pro!0} permission::android.permission.READ\_PHONE\_STATE & \cellcolor{pro!0} permission::android.permission.READ\_PHONE\_STATE \\
  28 & \cellcolor{con!7} api\_call::android/net/ConnectivityManager;-\textgreater{}getActiveNetworkInfo & \cellcolor{pro!0} api\_call::android/net/ConnectivityManager;-\textgreater{}getActiveNetworkInfo & \cellcolor{pro!0} api\_call::android/net/ConnectivityManager;-\textgreater{}getActiveNetworkInfo \\
  29 & \cellcolor{con!8} api\_call::android/net/wifi/WifiManager;-\textgreater{}getConnectionInfo & \cellcolor{pro!0} api\_call::android/net/wifi/WifiManager;-\textgreater{}getConnectionInfo & \cellcolor{pro!0} api\_call::android/net/wifi/WifiManager;-\textgreater{}getConnectionInfo \\
  30 & \cellcolor{con!11} api\_call::android/app/Activity;-\textgreater{}startActivity & \cellcolor{pro!0} api\_call::android/app/Activity;-\textgreater{}startActivity & \cellcolor{pro!0} api\_call::android/app/Activity;-\textgreater{}startActivity \\
  31 & \cellcolor{con!12} call::getDeviceId & \cellcolor{pro!0} call::getDeviceId & \cellcolor{pro!0} call::getDeviceId \\
  32 & \cellcolor{con!17} feature::android.hardware.wifi & \cellcolor{pro!0} feature::android.hardware.wifi & \cellcolor{pro!0} feature::android.hardware.wifi \\
  33 & \cellcolor{con!18} url::www.gstatic.com & \cellcolor{pro!100} url::www.gstatic.com & \cellcolor{pro!32} url::www.gstatic.com \\
  34 & \cellcolor{con!18} call::Cipher(AES/CBC/PKCS5Padding) & \cellcolor{pro!0} call::Cipher(AES/CBC/PKCS5Padding) & \cellcolor{pro!0} call::Cipher(AES/CBC/PKCS5Padding) \\
  35 & \cellcolor{con!20} url::http://www.gstatic.com/afma/sdk-core-v40.js\textbackslash{} & \cellcolor{pro!0} url::http://www.gstatic.com/afma/sdk-core-v40.js\textbackslash{} & \cellcolor{pro!0} url::http://www.gstatic.com/afma/sdk-core-v40.js\textbackslash{} \\
  36 & \cellcolor{con!21} permission::android.permission.ACCESS\_WIFI\_STATE & \cellcolor{pro!0} permission::android.permission.ACCESS\_WIFI\_STATE & \cellcolor{pro!0} permission::android.permission.ACCESS\_WIFI\_STATE \\
  37 & \cellcolor{con!23} permission::android.permission.WRITE\_EXTERNAL\_STORAGE & \cellcolor{pro!0} permission::android.permission.WRITE\_EXTERNAL\_STORAGE & \cellcolor{pro!0} permission::android.permission.WRITE\_EXTERNAL\_STORAGE \\
  38 & \cellcolor{con!49} api\_call::android/telephony/TelephonyManager;-\textgreater{}getDeviceId & \cellcolor{pro!0} api\_call::android/telephony/TelephonyManager;-\textgreater{}getDeviceId & \cellcolor{pro!0} api\_call::android/telephony/TelephonyManager;-\textgreater{}getDeviceId \\
  \bottomrule
\end{tabular}

==> tables/casestudy-damd-ig-lime.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \igShort & \bfseries \lime\\
  \midrule
  0 & \cellcolor{pro!4} \ttfamily invoke-virtual & \cellcolor{pro!44} \ttfamily invoke-virtual \\\\[ -3.5mm]
  1 & \cellcolor{pro!20} \ttfamily move-result-object & \cellcolor{con!5} \ttfamily move-result-object \\\\[ -3.5mm]
  2 & \cellcolor{pro!35} \ttfamily if-eqz & \cellcolor{pro!46} \ttfamily if-eqz \\\\[ -3.5mm]
  3 & \cellcolor{pro!25} \ttfamily const-string & \cellcolor{pro!35} \ttfamily const-string \\\\[ -3.5mm]
  4 & \cellcolor{pro!23} \ttfamily invoke-virtual & \cellcolor{pro!32} \ttfamily invoke-virtual \\\\[ -3.5mm]
  5 & \cellcolor{pro!13} \ttfamily move-result-object & \cellcolor{con!3} \ttfamily move-result-object \\\\[ -3.5mm]
  6 & \cellcolor{pro!44} \ttfamily check-cast & \cellcolor{pro!30} \ttfamily check-cast \\\\[ -3.5mm]
  7 & \cellcolor{pro!73} \ttfamily array-length & \cellcolor{pro!55} \ttfamily array-length \\\\[ -3.5mm]
  8 & \cellcolor{pro!42} \ttfamily new-array & \cellcolor{pro!1} \ttfamily new-array \\\\[ -3.5mm]
  9 & \cellcolor{pro!11} \ttfamily const/4 & \cellcolor{pro!19} \ttfamily const/4 \\\\[ -3.5mm]
  10 & \cellcolor{pro!6} \ttfamily array-length & \cellcolor{con!8} \ttfamily array-length \\\\[ -3.5mm]
  11 & \cellcolor{pro!11} \ttfamily if-ge & \cellcolor{pro!11} \ttfamily if-ge \\\\[ -3.5mm]
  12 & \cellcolor{pro!4} \ttfamily aget-object & \cellcolor{pro!12} \ttfamily aget-object \\\\[ -3.5mm]
  13 & \cellcolor{pro!5} \ttfamily check-cast & \cellcolor{con!18} \ttfamily check-cast \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-damd.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \lrp & \bfseries \lemna\\
  \midrule
  0 & \cellcolor{pro!7} \ttfamily invoke-virtual & \cellcolor{con!11} \ttfamily invoke-virtual \\\\[ -3.3mm]
  1 & \cellcolor{pro!27} \ttfamily move-result-object & \cellcolor{con!11} \ttfamily move-result-object \\\\[ -3.3mm]
  2 & \cellcolor{pro!48} \ttfamily if-eqz & \cellcolor{con!11} \ttfamily if-eqz \\\\[ -3.3mm]
  3 & \cellcolor{pro!33} \ttfamily const-string & \cellcolor{con!11} \ttfamily const-string \\\\[ -3.3mm]
  4 & \cellcolor{pro!28} \ttfamily invoke-virtual & \cellcolor{con!11} \ttfamily invoke-virtual \\\\[ -3.3mm]
  5 & \cellcolor{pro!17} \ttfamily move-result-object & \cellcolor{con!11} \ttfamily move-result-object \\\\[ -3.3mm]
  6 & \cellcolor{pro!56} \ttfamily check-cast & \cellcolor{con!11} \ttfamily check-cast \\\\[ -3.3mm]
  7 & \cellcolor{pro!99} \ttfamily array-length & \cellcolor{con!11} \ttfamily array-length \\\\[ -3.3mm]
  8 & \cellcolor{pro!48} \ttfamily new-array & \cellcolor{con!11} \ttfamily new-array \\\\[ -3.3mm]
  9 & \cellcolor{pro!13} \ttfamily const/4 & \cellcolor{con!11} \ttfamily const/4 \\\\[ -3.3mm]
  10 & \cellcolor{pro!5} \ttfamily array-length & \cellcolor{con!11} \ttfamily array-length \\\\[ -3.3mm]
  11 & \cellcolor{pro!14} \ttfamily if-ge & \cellcolor{con!11} \ttfamily if-ge \\\\[ -3.3mm]
  12 & \cellcolor{pro!6} \ttfamily aget-object & \cellcolor{con!10} \ttfamily aget-object \\\\[ -3.3mm]
  13 & \cellcolor{pro!7} \ttfamily check-cast & \cellcolor{con!10} \ttfamily check-cast \\\\[ -3.3mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-drebin-benign.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \lrp & \bfseries \lemna\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily feature::android.hardware.touchscreen & \cellcolor{pro!100} \ttfamily url::smartphone.solidam.com \\\\[ -3.5mm]
  1 & \cellcolor{pro!53} \ttfamily intent::android.intent.category.LAUNCHER & \cellcolor{pro!90} \ttfamily intent::android.intent.category.LAUNCHER \\\\[ -3.5mm]
  2 & \cellcolor{pro!24} \ttfamily real\_permission::android.permission.INTERNET & \cellcolor{pro!85} \ttfamily activity::.Settings \\\\[ -3.5mm]
  3 & \cellcolor{pro!23} \ttfamily api\_call::android/webkit/WebView & \cellcolor{pro!80} \ttfamily call::getSystemService \\\\[ -3.5mm]
  4 & \cellcolor{pro!23} \ttfamily call::Obfuscation(Base64) & \cellcolor{pro!73} \ttfamily api\_call::android/webkit/WebView \\\\[ -3.5mm]
  5 & \cellcolor{pro!19} \ttfamily feature::android.hardware.screen.portrait & \cellcolor{pro!69} \ttfamily activity::.ChoosePublication \\\\[ -3.5mm]
  6 & \cellcolor{pro!14} \ttfamily activity::.Settings & \cellcolor{pro!66} \ttfamily real\_permission::android.permission.INTERNET \\\\[ -3.5mm]
  7 & \cellcolor{pro!13} \ttfamily call::getSystemService & \cellcolor{pro!63} \ttfamily feature::android.hardware.screen.portrait \\\\[ -3.5mm]
  8 & \cellcolor{pro!9} \ttfamily permission::android.permission.INTERNET & \cellcolor{pro!61} \ttfamily activity::.WebView1 \\\\[ -3.5mm]
  9 & \cellcolor{pro!9} \ttfamily intent::android.intent.action.MAIN & \cellcolor{pro!59} \ttfamily permission::android.permission.VIBRATE \\\\[ -3.5mm]
  10 & \cellcolor{pro!8} \ttfamily permission::android.permission.ACCESS\_NETWORK\_STATE & \cellcolor{pro!50} \ttfamily real\_permission::android.permission.READ\_PHONE\_STATE \\\\[ -3.5mm]
  11 & \cellcolor{pro!7} \ttfamily real\_permission::android.permission.READ\_PHONE\_STATE & \cellcolor{pro!45} \ttfamily permission::android.permission.READ\_PHONE\_STATE \\\\[ -3.5mm]
  12 & \cellcolor{pro!3} \ttfamily activity::.ExpandableList1 & \cellcolor{pro!41} \ttfamily intent::android.intent.action.MAIN \\\\[ -3.5mm]
  13 & \cellcolor{pro!3} \ttfamily real\_permission::android.permission.ACCESS\_NETWORK\_STATE & \cellcolor{pro!37} \ttfamily activity::.ExpandableList1 \\\\[ -3.5mm]
  14 & \cellcolor{pro!1} \ttfamily activity::.ChoosePublication & \cellcolor{pro!37} \ttfamily permission::android.permission.INTERNET \\\\[ -3.5mm]
  15 & \cellcolor{pro!1} \ttfamily activity::.NewsViewer & \cellcolor{pro!34} \ttfamily permission::android.permission.ACCESS\_NETWORK\_STATE \\\\[ -3.5mm]
  16 & \cellcolor{pro!1} \ttfamily url::smartphone.solidam.com & \cellcolor{pro!34} \ttfamily activity::About \\\\[ -3.5mm]
  17 & \cellcolor{pro!0} \ttfamily url::http://smartphone.solidam.com/publications/demo/?phone\_id\%3D & \cellcolor{pro!31} \ttfamily call::printStackTrace \\\\[ -3.5mm]
  18 & \cellcolor{con!0} \ttfamily activity::.PageSelect & \cellcolor{pro!31} \ttfamily activity::.SectionBrowser \\\\[ -3.5mm]
  19 & \cellcolor{con!0} \ttfamily activity::.WebView1 & \cellcolor{pro!27} \ttfamily feature::android.hardware.touchscreen \\\\[ -3.5mm]
  20 & \cellcolor{con!1} \ttfamily permission::android.permission.READ\_PHONE\_STATE & \cellcolor{pro!19} \ttfamily url::http://smartphone.solidam.com/publications/demo/?phone\_id\%3D \\\\[ -3.5mm]
  21 & \cellcolor{con!1} \ttfamily call::printStackTrace & \cellcolor{pro!2} \ttfamily call::Obfuscation(Base64) \\\\[ -3.5mm]
  22 & \cellcolor{con!1} \ttfamily activity::.SectionBrowser & \cellcolor{con!1} \ttfamily api\_call::android/telephony/TelephonyManager;-\textgreater{}getDeviceId \\\\[ -3.5mm]
  23 & \cellcolor{con!10} \ttfamily call::getDeviceId & \cellcolor{con!9} \ttfamily real\_permission::android.permission.ACCESS\_NETWORK\_STATE \\\\[ -3.5mm]
  24 & \cellcolor{con!10} \ttfamily activity::About & \cellcolor{con!21} \ttfamily activity::.PageSelect \\\\[ -3.5mm]
  25 & \cellcolor{con!11} \ttfamily api\_call::android/net/ConnectivityManager;-\textgreater{}getActiveNetworkInfo & \cellcolor{con!24} \ttfamily call::getDeviceId \\\\[ -3.5mm]
  26 & \cellcolor{con!14} \ttfamily permission::android.permission.VIBRATE & \cellcolor{con!25} \ttfamily activity::.NewsViewer \\\\[ -3.5mm]
  27 & \cellcolor{con!48} \ttfamily api\_call::android/telephony/TelephonyManager;-\textgreater{}getDeviceId & \cellcolor{con!61} \ttfamily api\_call::android/net/ConnectivityManager;-\textgreater{}getActiveNetworkInfo \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-drebin-broken.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \lrp & \bfseries \lemna\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily feature::android.hardware.touchscreen & \cellcolor{pro!100} \ttfamily url::http://www.aga-love.org \\\\[ -3.5mm]
  1 & \cellcolor{pro!53} \ttfamily intent::android.intent.category.LAUNCHER & \cellcolor{pro!83} \ttfamily real\_permission::android.permission.RESTART\_PACKAGES \\\\[ -3.5mm]
  2 & \cellcolor{pro!23} \ttfamily real\_permission::android.permission.INTERNET & \cellcolor{pro!79} \ttfamily permission::android.permission.RESTART\_PACKAGES \\\\[ -3.5mm]
  3 & \cellcolor{pro!23} \ttfamily api\_call::android/webkit/WebView & \cellcolor{pro!74} \ttfamily activity::.Password \\\\[ -3.5mm]
  4 & \cellcolor{pro!20} \ttfamily feature::android.hardware.screen.portrait & \cellcolor{pro!61} \ttfamily intent::android.intent.category.LAUNCHER \\\\[ -3.5mm]
  5 & \cellcolor{pro!11} \ttfamily call::getSystemService & \cellcolor{pro!59} \ttfamily feature::android.hardware.touchscreen \\\\[ -3.5mm]
  6 & \cellcolor{pro!11} \ttfamily api\_call::android/app/ActivityManager;-\textgreater{}restartPackage & \cellcolor{pro!57} \ttfamily call::getSystemService \\\\[ -3.5mm]
  7 & \cellcolor{pro!10} \ttfamily real\_permission::android.permission.RESTART\_PACKAGES & \cellcolor{pro!56} \ttfamily url::www.aga-love.org \\\\[ -3.5mm]
  8 & \cellcolor{pro!10} \ttfamily permission::android.permission.INTERNET & \cellcolor{pro!56} \ttfamily api\_call::android/app/ActivityManager;-\textgreater{}restartPackage \\\\[ -3.5mm]
  9 & \cellcolor{pro!9} \ttfamily intent::android.intent.action.MAIN & \cellcolor{pro!54} \ttfamily url::www.agasarang.org \\\\[ -3.5mm]
  10 & \cellcolor{pro!0} \ttfamily url::http://www.agasarang.org & \cellcolor{pro!54} \ttfamily intent::android.intent.action.MAIN \\\\[ -3.5mm]
  11 & \cellcolor{pro!0} \ttfamily url::www.agasarang.org & \cellcolor{pro!48} \ttfamily real\_permission::android.permission.INTERNET \\\\[ -3.5mm]
  12 & \cellcolor{pro!0} \ttfamily activity::.Password & \cellcolor{pro!40} \ttfamily api\_call::android/webkit/WebView \\\\[ -3.5mm]
  13 & \cellcolor{pro!0} \ttfamily url::www.aga-love.org & \cellcolor{pro!31} \ttfamily url::http://www.agasarang.org \\\\[ -3.5mm]
  14 & \cellcolor{con!1} \ttfamily url::http://www.aga-love.org & \cellcolor{pro!25} \ttfamily feature::android.hardware.screen.portrait \\\\[ -3.5mm]
  15 & \cellcolor{con!12} \ttfamily permission::android.permission.RESTART\_PACKAGES & \cellcolor{pro!15} \ttfamily permission::android.permission.INTERNET \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-drebin-ig-lime.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \igShort & \bfseries \lime\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily permission::android.permission.SEND\_SMS & \cellcolor{pro!100} \ttfamily permission::android.permission.SEND\_SMS \\\\[ -3.5mm]
  1 & \cellcolor{pro!52} \ttfamily activity::.FirstActivity & \cellcolor{pro!59} \ttfamily call::sendSMS \\\\[ -3.5mm]
  2 & \cellcolor{pro!50} \ttfamily call::sendSMS & \cellcolor{pro!59} \ttfamily activity::.FirstActivity \\\\[ -3.5mm]
  3 & \cellcolor{pro!39} \ttfamily permission::android.permission.READ\_PHONE\_STATE & \cellcolor{pro!39} \ttfamily feature::android.hardware.telephony \\\\[ -3.5mm]
  4 & \cellcolor{pro!39} \ttfamily feature::android.hardware.telephony & \cellcolor{pro!37} \ttfamily intent::android.intent.action.DATA\_SMS\_RECEIVED \\\\[ -3.5mm]
  5 & \cellcolor{pro!38} \ttfamily intent::android.intent.action.DATA\_SMS\_RECEIVED & \cellcolor{pro!32} \ttfamily permission::android.permission.INTERNET \\\\[ -3.5mm]
  6 & \cellcolor{pro!37} \ttfamily service\_receiver::.services.SMSSenderService & \cellcolor{pro!26} \ttfamily permission::android.permission.READ\_PHONE\_STATE \\\\[ -3.5mm]
  7 & \cellcolor{pro!36} \ttfamily service\_receiver::.sms.BinarySMSReceiver & \cellcolor{pro!26} \ttfamily service\_receiver::.services.SMSSenderService \\\\[ -3.5mm]
  8 & \cellcolor{pro!30} \ttfamily permission::android.permission.INTERNET & \cellcolor{pro!25} \ttfamily call::getSimCountryIso \\\\[ -3.5mm]
  9 & \cellcolor{pro!30} \ttfamily call::getSimCountryIso & \cellcolor{pro!23} \ttfamily api\_call::android/../TelephonyManager;-\textgreater{}getLine1Number \\\\[ -3.5mm]
  10 & \cellcolor{pro!21} \ttfamily api\_call::android/../TelephonyManager;-\textgreater{}getLine1Number & \cellcolor{pro!18} \ttfamily api\_call::android/app/Activity;-\textgreater{}startActivity \\\\[ -3.5mm]
  11 & \cellcolor{pro!14} \ttfamily api\_call::android/app/Activity;-\textgreater{}startActivity & \cellcolor{pro!16} \ttfamily service\_receiver::.sms.BinarySMSReceiver \\\\[ -3.5mm]
  12 & \cellcolor{pro!10} \ttfamily permission::android.permission.RECEIVE\_SMS & \cellcolor{con!1} \ttfamily real\_permission::android.permission.SEND\_SMS \\\\[ -3.5mm]
  13 & \cellcolor{pro!7} \ttfamily real\_permission::android.permission.SEND\_SMS & \cellcolor{con!5} \ttfamily api\_call::org/apache/http/impl/client/DefaultHttpClient \\\\[ -3.5mm]
  14 & \cellcolor{pro!4} \ttfamily intent::android.intent.action.MAIN & \cellcolor{con!5} \ttfamily permission::android.permission.RECEIVE\_SMS \\\\[ -3.5mm]
  15 & \cellcolor{pro!0} \ttfamily call::printStackTrace & \cellcolor{con!5} \ttfamily call::printStackTrace \\\\[ -3.5mm]
  16 & \cellcolor{con!2} \ttfamily api\_call::org/apache/http/impl/client/DefaultHttpClient & \cellcolor{con!9} \ttfamily api\_call::android/telephony/SmsManager;-\textgreater{}sendTextMessage \\\\[ -3.5mm]
  17 & \cellcolor{con!7} \ttfamily api\_call::android/telephony/SmsManager;-\textgreater{}sendTextMessage & \cellcolor{con!14} \ttfamily real\_permission::android.permission.READ\_PHONE\_STATE \\\\[ -3.5mm]
  18 & \cellcolor{con!22} \ttfamily real\_permission::android.permission.READ\_PHONE\_STATE & \cellcolor{con!21} \ttfamily intent::android.intent.action.MAIN \\\\[ -3.5mm]
  19 & \cellcolor{con!29} \ttfamily call::getSystemService & \cellcolor{con!26} \ttfamily call::getSystemService \\\\[ -3.5mm]
  20 & \cellcolor{con!38} \ttfamily real\_permission::android.permission.INTERNET & \cellcolor{con!37} \ttfamily real\_permission::android.permission.INTERNET \\\\[ -3.5mm]
  21 & \cellcolor{con!66} \ttfamily intent::android.intent.category.LAUNCHER & \cellcolor{con!52} \ttfamily intent::android.intent.category.LAUNCHER \\\\[ -3.5mm]
  22 & \cellcolor{con!83} \ttfamily feature::android.hardware.touchscreen & \cellcolor{con!67} \ttfamily feature::android.hardware.touchscreen \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-drebin-ig.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \igLong \\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily permission::android.permission.SEND\_SMS \\\\[ -3.5mm]
  1 & \cellcolor{pro!52} \ttfamily activity::.FirstActivity \\\\[ -3.5mm]
  2 & \cellcolor{pro!50} \ttfamily call::sendSMS  \\\\[ -3.5mm]
  3 & \cellcolor{pro!39} \ttfamily permission::android.permission.READ\_PHONE\_STATE  \\\\[ -3.5mm]
  4 & \cellcolor{pro!39} \ttfamily feature::android.hardware.telephony \\\\[ -3.5mm]
  5 & \cellcolor{pro!38} \ttfamily intent::android.intent.action.DATA\_SMS\_RECEIVED \\\\[ -3.5mm]
  6 & \cellcolor{pro!37} \ttfamily service\_receiver::.services.SMSSenderService \\\\[ -3.5mm]
  7 & \cellcolor{pro!36} \ttfamily service\_receiver::.sms.BinarySMSReceiver \\\\[ -3.5mm]
  8 & \cellcolor{pro!30} \ttfamily permission::android.permission.INTERNET \\\\[ -3.5mm]
  9 & \cellcolor{pro!30} \ttfamily call::getSimCountryIso \\\\[ -3.5mm]
  10 & \cellcolor{pro!21} \ttfamily api\_call::android/../TelephonyManager;-\textgreater{}getLine1Number \\\\[ -3.5mm]
  11 & \cellcolor{pro!14} \ttfamily api\_call::android/app/Activity;-\textgreater{}startActivity \\\\[ -3.5mm]
  12 & \cellcolor{pro!10} \ttfamily permission::android.permission.RECEIVE\_SMS \\\\[ -3.5mm]
  13 & \cellcolor{pro!7} \ttfamily real\_permission::android.permission.SEND\_SMS \\\\[ -3.5mm]
  14 & \cellcolor{pro!4} \ttfamily intent::android.intent.action.MAIN \\\\[ -3.5mm]
  15 & \cellcolor{pro!0} \ttfamily call::printStackTrace \\\\[ -3.5mm]
  16 & \cellcolor{con!2} \ttfamily api\_call::org/apache/http/impl/client/DefaultHttpClient \\\\[ -3.5mm]
  17 & \cellcolor{con!7} \ttfamily api\_call::android/telephony/SmsManager;-\textgreater{}sendTextMessage \\\\[ -3.5mm]
  18 & \cellcolor{con!22} \ttfamily real\_permission::android.permission.READ\_PHONE\_STATE \\\\[ -3.5mm]
  19 & \cellcolor{con!29} \ttfamily call::getSystemService \\\\[ -3.5mm]
  20 & \cellcolor{con!38} \ttfamily real\_permission::android.permission.INTERNET \\\\[ -3.5mm]
  21 & \cellcolor{con!66} \ttfamily intent::android.intent.category.LAUNCHER \\\\[ -3.5mm]
  22 & \cellcolor{con!83} \ttfamily feature::android.hardware.touchscreen \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-drebin.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \lrp & \bfseries \lemna\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily permission::android.permission.SEND\_SMS & \cellcolor{pro!100} \ttfamily permission::android.permission.SEND\_SMS \\\\[ -3.5mm]
  1 & \cellcolor{pro!76} \ttfamily permission::android.permission.INTERNET & \cellcolor{pro!74} \ttfamily activity::.FirstActivity \\\\[ -3.5mm]
  2 & \cellcolor{pro!74} \ttfamily permission::android.permission.READ\_PHONE\_STATE & \cellcolor{pro!71} \ttfamily call::sendSMS \\\\[ -3.5mm]
  3 & \cellcolor{pro!69} \ttfamily activity::.FirstActivity & \cellcolor{pro!42} \ttfamily feature::android.hardware.telephony \\\\[ -3.5mm]
  4 & \cellcolor{pro!59} \ttfamily intent::android.intent.action.DATA\_SMS\_RECEIVED & \cellcolor{pro!36} \ttfamily permission::android.permission.INTERNET \\\\[ -3.5mm]
  5 & \cellcolor{pro!56} \ttfamily feature::android.hardware.telephony & \cellcolor{pro!36} \ttfamily intent::android.intent.action.DATA\_SMS\_RECEIVED \\\\[ -3.5mm]
  6 & \cellcolor{pro!50} \ttfamily service\_receiver::.services.SMSSenderService & \cellcolor{pro!29} \ttfamily call::getSimCountryIso \\\\[ -3.5mm]
  7 & \cellcolor{pro!47} \ttfamily service\_receiver::.sms.BinarySMSReceiver & \cellcolor{pro!28} \ttfamily permission::android.permission.READ\_PHONE\_STATE \\\\[ -3.5mm]
  8 & \cellcolor{pro!42} \ttfamily call::getSimCountryIso & \cellcolor{pro!26} \ttfamily service\_receiver::.sms.BinarySMSReceiver \\\\[ -3.5mm]
  9 & \cellcolor{pro!35} \ttfamily call::sendSMS & \cellcolor{pro!25} \ttfamily api\_call::android/app/Activity;-\textgreater{}startActivity \\\\[ -3.5mm]
  10 & \cellcolor{pro!30} \ttfamily permission::android.permission.RECEIVE\_SMS & \cellcolor{pro!25} \ttfamily service\_receiver::.services.SMSSenderService \\\\[ -3.5mm]
  11 & \cellcolor{pro!19} \ttfamily intent::android.intent.action.MAIN & \cellcolor{pro!21} \ttfamily api\_call::.../TelephonyManager;-\textgreater{}getLine1Number \\\\[ -3.5mm]
  12 & \cellcolor{pro!18} \ttfamily api\_call::.../TelephonyManager;-\textgreater{}getLine1Number & \cellcolor{pro!14} \ttfamily real\_permission::android.permission.SEND\_SMS \\\\[ -3.5mm]
  13 & \cellcolor{pro!12} \ttfamily api\_call::android/app/Activity;-\textgreater{}startActivity & \cellcolor{pro!9} \ttfamily api\_call::android/telephony/SmsManager;-\textgreater{}sendTextMessage \\\\[ -3.5mm]
  14 & \cellcolor{pro!4} \ttfamily api\_call::org/apache/http/impl/client/DefaultHttpClient & \cellcolor{pro!6} \ttfamily api\_call::org/apache/http/impl/client/DefaultHttpClient \\\\[ -3.5mm]
  15 & \cellcolor{con!2} \ttfamily api\_call::android/telephony/SmsManager;-\textgreater{}sendTextMessage & \cellcolor{pro!6} \ttfamily call::printStackTrace \\\\[ -3.5mm]
  16 & \cellcolor{con!5} \ttfamily call::printStackTrace & \cellcolor{con!3} \ttfamily permission::android.permission.RECEIVE\_SMS \\\\[ -3.5mm]
  17 & \cellcolor{con!15} \ttfamily real\_permission::android.permission.SEND\_SMS & \cellcolor{con!4} \ttfamily real\_permission::android.permission.READ\_PHONE\_STATE \\\\[ -3.5mm]
  18 & \cellcolor{con!23} \ttfamily feature::android.hardware.touchscreen & \cellcolor{con!14} \ttfamily call::getSystemService \\\\[ -3.5mm]
  19 & \cellcolor{con!34} \ttfamily real\_permission::android.permission.READ\_PHONE\_STATE & \cellcolor{con!15} \ttfamily intent::android.intent.action.MAIN \\\\[ -3.5mm]
  20 & \cellcolor{con!45} \ttfamily call::getSystemService & \cellcolor{con!37} \ttfamily real\_permission::android.permission.INTERNET \\\\[ -3.5mm]
  21 & \cellcolor{con!48} \ttfamily real\_permission::android.permission.INTERNET & \cellcolor{con!41} \ttfamily intent::android.intent.category.LAUNCHER \\\\[ -3.5mm]
  22 & \cellcolor{con!48} \ttfamily intent::android.intent.category.LAUNCHER & \cellcolor{con!68} \ttfamily feature::android.hardware.touchscreen \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-mimicus-ig-lime-shortened.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \igShort & \bfseries \lime\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily \ttfamily count\_javascript & \cellcolor{pro!100} \ttfamily \ttfamily count\_js \\\\[ -3.5mm]
  1 & \cellcolor{pro!79} \ttfamily count\_js & \cellcolor{pro!88} \ttfamily count\_javascript \\\\[ -3.5mm]
  2 & \cellcolor{pro!17} \ttfamily count\_trailer & \cellcolor{pro!39} \ttfamily count\_page \\\\[ -3.5mm]
  3 & \cellcolor{pro!14} \ttfamily count\_endobj & \cellcolor{pro!38} \ttfamily ratio\_size\_stream \\\\[ -3.5mm]
  4 & \cellcolor{pro!12} \ttfamily box\_other\_only & \cellcolor{pro!35} \ttfamily createdate\_version\_ratio \\\\[ -3.5mm]
  5 & \cellcolor{pro!10} \ttfamily pos\_page\_avg & \cellcolor{pro!32} \ttfamily size \\\\[ -3.5mm]
  6 & \cellcolor{pro!9} \ttfamily createdate\_tz & \cellcolor{pro!32} \ttfamily createdate\_tz \\\\[ -3.5mm]
  7 & \cellcolor{pro!8} \ttfamily count\_stream & \cellcolor{pro!31} \ttfamily pos\_acroform\_avg \\\\[ -3.5mm]
  8 & \cellcolor{pro!8} \ttfamily pos\_page\_min & \cellcolor{pro!27} \ttfamily pos\_box\_min \\\\[ -3.5mm]
  9 & \cellcolor{pro!7} \ttfamily ratio\_size\_stream & \cellcolor{pro!24} \ttfamily pos\_page\_min \\\\[ -3.5mm]
  10 & \cellcolor{pro!0} \ttfamily ... & \cellcolor{pro!0} \ttfamily ... \\\\[ -3.5mm]
  34 & \cellcolor{con!3} \ttfamily moddate\_tz & \cellcolor{con!12} \ttfamily pos\_page\_avg \\\\[ -3.5mm]
  35 & \cellcolor{con!4} \ttfamily size & \cellcolor{con!12} \ttfamily pos\_image\_avg \\\\[ -3.5mm]
  36 & \cellcolor{con!5} \ttfamily pos\_eof\_max & \cellcolor{con!15} \ttfamily pos\_eof\_avg \\\\[ -3.5mm]
  37 & \cellcolor{con!8} \ttfamily count\_endstream & \cellcolor{con!15} \ttfamily pos\_image\_min \\\\[ -3.5mm]
  38 & \cellcolor{con!8} \ttfamily pos\_eof\_avg & \cellcolor{con!18} \ttfamily ratio\_size\_page \\\\[ -3.5mm]
  39 & \cellcolor{con!9} \ttfamily moddate\_version\_ratio & \cellcolor{con!20} \ttfamily count\_eof \\\\[ -3.5mm]
  40 & \cellcolor{con!10} \ttfamily count\_xref & \cellcolor{con!24} \ttfamily len\_stream\_max \\\\[ -3.5mm]
  41 & \cellcolor{con!14} \ttfamily count\_eof & \cellcolor{con!29} \ttfamily moddate\_tz \\\\[ -3.5mm]
  42 & \cellcolor{con!17} \ttfamily pos\_eof\_min & \cellcolor{con!31} \ttfamily count\_xref \\\\[ -3.5mm]
  43 & \cellcolor{con!17} \ttfamily len\_stream\_max & \cellcolor{con!43} \ttfamily pos\_eof\_min \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-mimicus-ig-lime.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \igShort & \bfseries \lime\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily count\_javascript & \cellcolor{pro!100} \ttfamily count\_js \\\\[ -3.5mm]
  1 & \cellcolor{pro!79} \ttfamily count\_js & \cellcolor{pro!88} \ttfamily count\_javascript \\\\[ -3.5mm]
  2 & \cellcolor{pro!17} \ttfamily count\_trailer & \cellcolor{pro!39} \ttfamily count\_page \\\\[ -3.5mm]
  3 & \cellcolor{pro!14} \ttfamily count\_endobj & \cellcolor{pro!38} \ttfamily ratio\_size\_stream \\\\[ -3.5mm]
  4 & \cellcolor{pro!12} \ttfamily box\_other\_only & \cellcolor{pro!35} \ttfamily createdate\_version\_ratio \\\\[ -3.5mm]
  5 & \cellcolor{pro!10} \ttfamily pos\_page\_avg & \cellcolor{pro!32} \ttfamily size \\\\[ -3.5mm]
  6 & \cellcolor{pro!9} \ttfamily createdate\_tz & \cellcolor{pro!32} \ttfamily createdate\_tz \\\\[ -3.5mm]
  7 & \cellcolor{pro!8} \ttfamily count\_stream & \cellcolor{pro!31} \ttfamily pos\_acroform\_avg \\\\[ -3.5mm]
  8 & \cellcolor{pro!8} \ttfamily pos\_page\_min & \cellcolor{pro!27} \ttfamily pos\_box\_min \\\\[ -3.5mm]
  9 & \cellcolor{pro!7} \ttfamily ratio\_size\_stream & \cellcolor{pro!24} \ttfamily pos\_page\_min \\\\[ -3.5mm]
  10 & \cellcolor{pro!6} \ttfamily len\_obj\_min & \cellcolor{pro!24} \ttfamily pos\_box\_max \\\\[ -3.5mm]
  11 & \cellcolor{pro!6} \ttfamily count\_page & \cellcolor{pro!18} \ttfamily count\_stream \\\\[ -3.5mm]
  12 & \cellcolor{pro!6} \ttfamily pos\_box\_avg & \cellcolor{pro!17} \ttfamily pos\_page\_max \\\\[ -3.5mm]
  13 & \cellcolor{pro!5} \ttfamily pos\_page\_max & \cellcolor{pro!17} \ttfamily version \\\\[ -3.5mm]
  14 & \cellcolor{pro!5} \ttfamily pos\_acroform\_min & \cellcolor{pro!14} \ttfamily pos\_acroform\_min \\\\[ -3.5mm]
  15 & \cellcolor{pro!4} \ttfamily pos\_acroform\_avg & \cellcolor{pro!14} \ttfamily len\_stream\_min \\\\[ -3.5mm]
  16 & \cellcolor{pro!4} \ttfamily moddate\_ts & \cellcolor{pro!13} \ttfamily len\_obj\_avg \\\\[ -3.5mm]
  17 & \cellcolor{pro!3} \ttfamily pos\_image\_max & \cellcolor{pro!11} \ttfamily pos\_image\_max \\\\[ -3.5mm]
  18 & \cellcolor{pro!3} \ttfamily pos\_box\_min & \cellcolor{pro!9} \ttfamily createdate\_ts \\\\[ -3.5mm]
  19 & \cellcolor{pro!3} \ttfamily pos\_image\_avg & \cellcolor{pro!9} \ttfamily count\_obj \\\\[ -3.5mm]
  20 & \cellcolor{pro!3} \ttfamily len\_obj\_max & \cellcolor{pro!9} \ttfamily ratio\_size\_obj \\\\[ -3.5mm]
  21 & \cellcolor{pro!3} \ttfamily createdate\_ts & \cellcolor{pro!9} \ttfamily count\_trailer \\\\[ -3.5mm]
  22 & \cellcolor{pro!2} \ttfamily pos\_box\_max & \cellcolor{pro!8} \ttfamily pos\_eof\_max \\\\[ -3.5mm]
  23 & \cellcolor{pro!2} \ttfamily ratio\_size\_page & \cellcolor{pro!5} \ttfamily box\_other\_only \\\\[ -3.5mm]
  24 & \cellcolor{pro!1} \ttfamily len\_stream\_min & \cellcolor{pro!4} \ttfamily len\_obj\_max \\\\[ -3.5mm]
  25 & \cellcolor{pro!1} \ttfamily pos\_acroform\_max & \cellcolor{pro!4} \ttfamily pos\_acroform\_max \\\\[ -3.5mm]
  26 & \cellcolor{pro!1} \ttfamily count\_obj & \cellcolor{pro!3} \ttfamily pos\_box\_avg \\\\[ -3.5mm]
  27 & \cellcolor{con!1} \ttfamily createdate\_version\_ratio & \cellcolor{pro!2} \ttfamily len\_obj\_min \\\\[ -3.5mm]
  28 & \cellcolor{con!1} \ttfamily len\_obj\_avg & \cellcolor{pro!1} \ttfamily count\_endobj \\\\[ -3.5mm]
  29 & \cellcolor{con!1} \ttfamily count\_startxref & \cellcolor{pro!0} \ttfamily moddate\_ts \\\\[ -3.5mm]
  30 & \cellcolor{con!1} \ttfamily ratio\_size\_obj & \cellcolor{con!0} \ttfamily len\_stream\_avg \\\\[ -3.5mm]
  31 & \cellcolor{con!2} \ttfamily pos\_image\_min & \cellcolor{con!3} \ttfamily moddate\_version\_ratio \\\\[ -3.5mm]
  32 & \cellcolor{con!2} \ttfamily len\_stream\_avg & \cellcolor{con!9} \ttfamily count\_startxref \\\\[ -3.5mm]
  33 & \cellcolor{con!2} \ttfamily version & \cellcolor{con!12} \ttfamily count\_endstream \\\\[ -3.5mm]
  34 & \cellcolor{con!3} \ttfamily moddate\_tz & \cellcolor{con!12} \ttfamily pos\_page\_avg \\\\[ -3.5mm]
  35 & \cellcolor{con!4} \ttfamily size & \cellcolor{con!12} \ttfamily pos\_image\_avg \\\\[ -3.5mm]
  36 & \cellcolor{con!5} \ttfamily pos\_eof\_max & \cellcolor{con!15} \ttfamily pos\_eof\_avg \\\\[ -3.5mm]
  37 & \cellcolor{con!8} \ttfamily count\_endstream & \cellcolor{con!15} \ttfamily pos\_image\_min \\\\[ -3.5mm]
  38 & \cellcolor{con!8} \ttfamily pos\_eof\_avg & \cellcolor{con!18} \ttfamily ratio\_size\_page \\\\[ -3.5mm]
  39 & \cellcolor{con!9} \ttfamily moddate\_version\_ratio & \cellcolor{con!20} \ttfamily count\_eof \\\\[ -3.5mm]
  40 & \cellcolor{con!10} \ttfamily count\_xref & \cellcolor{con!24} \ttfamily len\_stream\_max \\\\[ -3.5mm]
  41 & \cellcolor{con!14} \ttfamily count\_eof & \cellcolor{con!29} \ttfamily moddate\_tz \\\\[ -3.5mm]
  42 & \cellcolor{con!17} \ttfamily pos\_eof\_min & \cellcolor{con!31} \ttfamily count\_xref \\\\[ -3.5mm]
  43 & \cellcolor{con!17} \ttfamily len\_stream\_max & \cellcolor{con!43} \ttfamily pos\_eof\_min \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-mimicus-ig-shortened.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \igLong\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily \ttfamily count\_javascript \\\\[ -3.5mm]
  1 & \cellcolor{pro!79} \ttfamily count\_js \\\\[ -3.5mm]
  2 & \cellcolor{pro!17} \ttfamily count\_trailer \\\\[ -3.5mm]
  3 & \cellcolor{pro!14} \ttfamily count\_endobj \\\\[ -3.5mm]
  4 & \cellcolor{pro!12} \ttfamily box\_other\_only \\\\[ -3.5mm]
  5 & \cellcolor{pro!10} \ttfamily pos\_page\_avg \\\\[ -3.5mm]
  6 & \cellcolor{pro!9} \ttfamily createdate\_tz \\\\[ -3.5mm]
  7 & \cellcolor{pro!8} \ttfamily count\_stream \\\\[ -3.5mm]
  8 & \cellcolor{pro!8} \ttfamily pos\_page\_min \\\\[ -3.5mm]
  9 & \cellcolor{pro!7} \ttfamily ratio\_size\_stream \\\\[ -3.5mm]
  10 & \cellcolor{pro!0} \ttfamily ... \\\\[ -3.5mm]
  34 & \cellcolor{con!3} \ttfamily moddate\_tz \\\\[ -3.5mm]
  35 & \cellcolor{con!4} \ttfamily size \\\\[ -3.5mm]
  36 & \cellcolor{con!5} \ttfamily pos\_eof\_max \\\\[ -3.5mm]
  37 & \cellcolor{con!8} \ttfamily count\_endstream \\\\[ -3.5mm]
  38 & \cellcolor{con!8} \ttfamily pos\_eof\_avg \\\\[ -3.5mm]
  39 & \cellcolor{con!9} \ttfamily moddate\_version\_ratio \\\\[ -3.5mm]
  40 & \cellcolor{con!10} \ttfamily count\_xref \\\\[ -3.5mm]
  41 & \cellcolor{con!14} \ttfamily count\_eof \\\\[ -3.5mm]
  42 & \cellcolor{con!17} \ttfamily pos\_eof\_min \\\\[ -3.5mm]
  43 & \cellcolor{con!17} \ttfamily len\_stream\_max \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-mimicus-no-stability.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries lemna_1 & \bfseries lemna_2\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily pos\_page\_min & \cellcolor{pro!4} \ttfamily pos\_page\_min \\\\[ -3.5mm]
  1 & \cellcolor{pro!94} \ttfamily count\_js & \cellcolor{pro!56} \ttfamily count\_js \\\\[ -3.5mm]
  2 & \cellcolor{pro!77} \ttfamily count\_javascript & \cellcolor{pro!22} \ttfamily count\_javascript \\\\[ -3.5mm]
  3 & \cellcolor{pro!72} \ttfamily pos\_acroform\_min & \cellcolor{pro!35} \ttfamily pos\_acroform\_min \\\\[ -3.5mm]
  4 & \cellcolor{pro!69} \ttfamily ratio\_size\_page & \cellcolor{pro!66} \ttfamily ratio\_size\_page \\\\[ -3.5mm]
  5 & \cellcolor{pro!66} \ttfamily pos\_image\_min & \cellcolor{pro!12} \ttfamily pos\_image\_min \\\\[ -3.5mm]
  6 & \cellcolor{pro!66} \ttfamily count\_obj & \cellcolor{con!5} \ttfamily count\_obj \\\\[ -3.5mm]
  7 & \cellcolor{pro!64} \ttfamily pos\_box\_avg & \cellcolor{pro!12} \ttfamily pos\_box\_avg \\\\[ -3.5mm]
  8 & \cellcolor{pro!60} \ttfamily createdate\_tz & \cellcolor{pro!11} \ttfamily createdate\_tz \\\\[ -3.5mm]
  9 & \cellcolor{pro!58} \ttfamily pos\_image\_avg & \cellcolor{pro!7} \ttfamily pos\_image\_avg \\\\[ -3.5mm]
  10 & \cellcolor{pro!55} \ttfamily len\_obj\_avg & \cellcolor{pro!100} \ttfamily len\_obj\_avg \\\\[ -3.5mm]
  11 & \cellcolor{pro!54} \ttfamily len\_stream\_min & \cellcolor{pro!33} \ttfamily len\_stream\_min \\\\[ -3.5mm]
  12 & \cellcolor{pro!51} \ttfamily box\_other\_only & \cellcolor{pro!2} \ttfamily box\_other\_only \\\\[ -3.5mm]
  13 & \cellcolor{pro!49} \ttfamily moddate\_ts & \cellcolor{pro!78} \ttfamily moddate\_ts \\\\[ -3.5mm]
  14 & \cellcolor{pro!47} \ttfamily pos\_acroform\_avg & \cellcolor{con!10} \ttfamily pos\_acroform\_avg \\\\[ -3.5mm]
  15 & \cellcolor{pro!47} \ttfamily pos\_acroform\_max & \cellcolor{pro!26} \ttfamily pos\_acroform\_max \\\\[ -3.5mm]
  16 & \cellcolor{pro!45} \ttfamily count\_trailer & \cellcolor{pro!58} \ttfamily count\_trailer \\\\[ -3.5mm]
  17 & \cellcolor{pro!44} \ttfamily pos\_box\_max & \cellcolor{pro!20} \ttfamily pos\_box\_max \\\\[ -3.5mm]
  18 & \cellcolor{pro!42} \ttfamily len\_obj\_min & \cellcolor{pro!90} \ttfamily len\_obj\_min \\\\[ -3.5mm]
  19 & \cellcolor{pro!39} \ttfamily createdate\_ts & \cellcolor{pro!56} \ttfamily createdate\_ts \\\\[ -3.5mm]
  20 & \cellcolor{pro!37} \ttfamily pos\_page\_max & \cellcolor{pro!23} \ttfamily pos\_page\_max \\\\[ -3.5mm]
  21 & \cellcolor{pro!36} \ttfamily pos\_box\_min & \cellcolor{pro!83} \ttfamily pos\_box\_min \\\\[ -3.5mm]
  22 & \cellcolor{pro!29} \ttfamily size & \cellcolor{pro!60} \ttfamily size \\\\[ -3.5mm]
  23 & \cellcolor{pro!28} \ttfamily ratio\_size\_stream & \cellcolor{pro!51} \ttfamily ratio\_size\_stream \\\\[ -3.5mm]
  24 & \cellcolor{pro!25} \ttfamily len\_obj\_max & \cellcolor{con!20} \ttfamily len\_obj\_max \\\\[ -3.5mm]
  25 & \cellcolor{pro!21} \ttfamily count\_endobj & \cellcolor{con!20} \ttfamily count\_endobj \\\\[ -3.5mm]
  26 & \cellcolor{pro!18} \ttfamily ratio\_size\_obj & \cellcolor{pro!22} \ttfamily ratio\_size\_obj \\\\[ -3.5mm]
  27 & \cellcolor{pro!16} \ttfamily pos\_image\_max & \cellcolor{pro!17} \ttfamily pos\_image\_max \\\\[ -3.5mm]
  28 & \cellcolor{pro!15} \ttfamily count\_page & \cellcolor{pro!78} \ttfamily count\_page \\\\[ -3.5mm]
  29 & \cellcolor{pro!14} \ttfamily len\_stream\_avg & \cellcolor{pro!72} \ttfamily len\_stream\_avg \\\\[ -3.5mm]
  30 & \cellcolor{pro!12} \ttfamily pos\_page\_avg & \cellcolor{pro!51} \ttfamily pos\_page\_avg \\\\[ -3.5mm]
  31 & \cellcolor{pro!10} \ttfamily count\_stream & \cellcolor{pro!18} \ttfamily count\_stream \\\\[ -3.5mm]
  32 & \cellcolor{con!9} \ttfamily moddate\_tz & \cellcolor{con!4} \ttfamily moddate\_tz \\\\[ -3.5mm]
  33 & \cellcolor{con!65} \ttfamily len\_stream\_max & \cellcolor{con!23} \ttfamily len\_stream\_max \\\\[ -3.5mm]
  34 & \cellcolor{con!100} \ttfamily count\_endstream & \cellcolor{pro!7} \ttfamily count\_endstream \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-mimicus-shortened.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \lrp & \bfseries \lemna\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily count\_javascript & \cellcolor{pro!100} \ttfamily count\_js \\\\[ -3.5mm]
  1 & \cellcolor{pro!79} \ttfamily count\_js & \cellcolor{pro!88} \ttfamily count\_javascript \\\\[ -3.5mm]
  2 & \cellcolor{pro!17} \ttfamily count\_trailer & \cellcolor{pro!39} \ttfamily count\_page \\\\[ -3.5mm]
  3 & \cellcolor{pro!14} \ttfamily count\_endobj & \cellcolor{pro!38} \ttfamily ratio\_size\_stream \\\\[ -3.5mm]
  4 & \cellcolor{pro!12} \ttfamily box\_other\_only & \cellcolor{pro!35} \ttfamily createdate\_version\_ratio \\\\[ -3.5mm]
  5 & \cellcolor{pro!10} \ttfamily pos\_page\_avg & \cellcolor{pro!32} \ttfamily size \\\\[ -3.5mm]
  6 & \cellcolor{pro!9} \ttfamily createdate\_tz & \cellcolor{pro!32} \ttfamily createdate\_tz \\\\[ -3.5mm]
  7 & \cellcolor{pro!8} \ttfamily count\_stream & \cellcolor{pro!31} \ttfamily pos\_acroform\_avg \\\\[ -3.5mm]
  8 & \cellcolor{pro!8} \ttfamily pos\_page\_min & \cellcolor{pro!27} \ttfamily pos\_box\_min \\\\[ -3.5mm]
  9 & \cellcolor{pro!7} \ttfamily ratio\_size\_stream & \cellcolor{pro!24} \ttfamily pos\_page\_min \\\\[ -3.5mm]
  10 & \cellcolor{pro!0} \ttfamily ... & \cellcolor{pro!0} \ttfamily ... \\\\[ -3.5mm]
  34 & \cellcolor{con!3} \ttfamily moddate\_tz & \cellcolor{con!12} \ttfamily pos\_page\_avg \\\\[ -3.5mm]
  35 & \cellcolor{con!4} \ttfamily size & \cellcolor{con!12} \ttfamily pos\_image\_avg \\\\[ -3.5mm]
  36 & \cellcolor{con!5} \ttfamily pos\_eof\_max & \cellcolor{con!15} \ttfamily pos\_eof\_avg \\\\[ -3.5mm]
  37 & \cellcolor{con!8} \ttfamily count\_endstream & \cellcolor{con!15} \ttfamily pos\_image\_min \\\\[ -3.5mm]
  38 & \cellcolor{con!8} \ttfamily pos\_eof\_avg & \cellcolor{con!18} \ttfamily ratio\_size\_page \\\\[ -3.5mm]
  39 & \cellcolor{con!9} \ttfamily moddate\_version\_ratio & \cellcolor{con!20} \ttfamily count\_eof \\\\[ -3.5mm]
  40 & \cellcolor{con!10} \ttfamily count\_xref & \cellcolor{con!24} \ttfamily len\_stream\_max \\\\[ -3.5mm]
  41 & \cellcolor{con!14} \ttfamily count\_eof & \cellcolor{con!29} \ttfamily moddate\_tz \\\\[ -3.5mm]
  42 & \cellcolor{con!17} \ttfamily pos\_eof\_min & \cellcolor{con!31} \ttfamily count\_xref \\\\[ -3.5mm]
  43 & \cellcolor{con!17} \ttfamily len\_stream\_max & \cellcolor{con!43} \ttfamily pos\_eof\_min \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-mimicus.tex <==
\begin{tabular}{
  cl@{\hskip 0.2in}l
}
  \toprule
  \bfseries Id & \bfseries \lrp & \bfseries \lemna\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily count\_javascript & \cellcolor{pro!100} \ttfamily count\_js \\\\[ -3.5mm]
  1 & \cellcolor{pro!79} \ttfamily count\_js & \cellcolor{pro!88} \ttfamily count\_javascript \\\\[ -3.5mm]
  2 & \cellcolor{pro!17} \ttfamily count\_trailer & \cellcolor{pro!39} \ttfamily count\_page \\\\[ -3.5mm]
  3 & \cellcolor{pro!14} \ttfamily count\_endobj & \cellcolor{pro!38} \ttfamily ratio\_size\_stream \\\\[ -3.5mm]
  4 & \cellcolor{pro!12} \ttfamily box\_other\_only & \cellcolor{pro!35} \ttfamily createdate\_version\_ratio \\\\[ -3.5mm]
  5 & \cellcolor{pro!10} \ttfamily pos\_page\_avg & \cellcolor{pro!32} \ttfamily size \\\\[ -3.5mm]
  6 & \cellcolor{pro!9} \ttfamily createdate\_tz & \cellcolor{pro!32} \ttfamily createdate\_tz \\\\[ -3.5mm]
  7 & \cellcolor{pro!8} \ttfamily count\_stream & \cellcolor{pro!31} \ttfamily pos\_acroform\_avg \\\\[ -3.5mm]
  8 & \cellcolor{pro!8} \ttfamily pos\_page\_min & \cellcolor{pro!27} \ttfamily pos\_box\_min \\\\[ -3.5mm]
  9 & \cellcolor{pro!7} \ttfamily ratio\_size\_stream & \cellcolor{pro!24} \ttfamily pos\_page\_min \\\\[ -3.5mm]
  10 & \cellcolor{pro!6} \ttfamily len\_obj\_min & \cellcolor{pro!24} \ttfamily pos\_box\_max \\\\[ -3.5mm]
  11 & \cellcolor{pro!6} \ttfamily count\_page & \cellcolor{pro!18} \ttfamily count\_stream \\\\[ -3.5mm]
  12 & \cellcolor{pro!6} \ttfamily pos\_box\_avg & \cellcolor{pro!17} \ttfamily pos\_page\_max \\\\[ -3.5mm]
  13 & \cellcolor{pro!5} \ttfamily pos\_page\_max & \cellcolor{pro!17} \ttfamily version \\\\[ -3.5mm]
  14 & \cellcolor{pro!5} \ttfamily pos\_acroform\_min & \cellcolor{pro!14} \ttfamily pos\_acroform\_min \\\\[ -3.5mm]
  15 & \cellcolor{pro!4} \ttfamily pos\_acroform\_avg & \cellcolor{pro!14} \ttfamily len\_stream\_min \\\\[ -3.5mm]
  16 & \cellcolor{pro!4} \ttfamily moddate\_ts & \cellcolor{pro!13} \ttfamily len\_obj\_avg \\\\[ -3.5mm]
  17 & \cellcolor{pro!3} \ttfamily pos\_image\_max & \cellcolor{pro!11} \ttfamily pos\_image\_max \\\\[ -3.5mm]
  18 & \cellcolor{pro!3} \ttfamily pos\_box\_min & \cellcolor{pro!9} \ttfamily createdate\_ts \\\\[ -3.5mm]
  19 & \cellcolor{pro!3} \ttfamily pos\_image\_avg & \cellcolor{pro!9} \ttfamily count\_obj \\\\[ -3.5mm]
  20 & \cellcolor{pro!3} \ttfamily len\_obj\_max & \cellcolor{pro!9} \ttfamily ratio\_size\_obj \\\\[ -3.5mm]
  21 & \cellcolor{pro!3} \ttfamily createdate\_ts & \cellcolor{pro!9} \ttfamily count\_trailer \\\\[ -3.5mm]
  22 & \cellcolor{pro!2} \ttfamily pos\_box\_max & \cellcolor{pro!8} \ttfamily pos\_eof\_max \\\\[ -3.5mm]
  23 & \cellcolor{pro!2} \ttfamily ratio\_size\_page & \cellcolor{pro!5} \ttfamily box\_other\_only \\\\[ -3.5mm]
  24 & \cellcolor{pro!1} \ttfamily len\_stream\_min & \cellcolor{pro!4} \ttfamily len\_obj\_max \\\\[ -3.5mm]
  25 & \cellcolor{pro!1} \ttfamily pos\_acroform\_max & \cellcolor{pro!4} \ttfamily pos\_acroform\_max \\\\[ -3.5mm]
  26 & \cellcolor{pro!1} \ttfamily count\_obj & \cellcolor{pro!3} \ttfamily pos\_box\_avg \\\\[ -3.5mm]
  27 & \cellcolor{con!1} \ttfamily createdate\_version\_ratio & \cellcolor{pro!2} \ttfamily len\_obj\_min \\\\[ -3.5mm]
  28 & \cellcolor{con!1} \ttfamily len\_obj\_avg & \cellcolor{pro!1} \ttfamily count\_endobj \\\\[ -3.5mm]
  29 & \cellcolor{con!1} \ttfamily count\_startxref & \cellcolor{pro!0} \ttfamily moddate\_ts \\\\[ -3.5mm]
  30 & \cellcolor{con!1} \ttfamily ratio\_size\_obj & \cellcolor{con!0} \ttfamily len\_stream\_avg \\\\[ -3.5mm]
  31 & \cellcolor{con!2} \ttfamily pos\_image\_min & \cellcolor{con!3} \ttfamily moddate\_version\_ratio \\\\[ -3.5mm]
  32 & \cellcolor{con!2} \ttfamily len\_stream\_avg & \cellcolor{con!9} \ttfamily count\_startxref \\\\[ -3.5mm]
  33 & \cellcolor{con!2} \ttfamily version & \cellcolor{con!12} \ttfamily count\_endstream \\\\[ -3.5mm]
  34 & \cellcolor{con!3} \ttfamily moddate\_tz & \cellcolor{con!12} \ttfamily pos\_page\_avg \\\\[ -3.5mm]
  35 & \cellcolor{con!4} \ttfamily size & \cellcolor{con!12} \ttfamily pos\_image\_avg \\\\[ -3.5mm]
  36 & \cellcolor{con!5} \ttfamily pos\_eof\_max & \cellcolor{con!15} \ttfamily pos\_eof\_avg \\\\[ -3.5mm]
  37 & \cellcolor{con!8} \ttfamily count\_endstream & \cellcolor{con!15} \ttfamily pos\_image\_min \\\\[ -3.5mm]
  38 & \cellcolor{con!8} \ttfamily pos\_eof\_avg & \cellcolor{con!18} \ttfamily ratio\_size\_page \\\\[ -3.5mm]
  39 & \cellcolor{con!9} \ttfamily moddate\_version\_ratio & \cellcolor{con!20} \ttfamily count\_eof \\\\[ -3.5mm]
  40 & \cellcolor{con!10} \ttfamily count\_xref & \cellcolor{con!24} \ttfamily len\_stream\_max \\\\[ -3.5mm]
  41 & \cellcolor{con!14} \ttfamily count\_eof & \cellcolor{con!29} \ttfamily moddate\_tz \\\\[ -3.5mm]
  42 & \cellcolor{con!17} \ttfamily pos\_eof\_min & \cellcolor{con!31} \ttfamily count\_xref \\\\[ -3.5mm]
  43 & \cellcolor{con!17} \ttfamily len\_stream\_max & \cellcolor{con!43} \ttfamily pos\_eof\_min \\\\[ -3.5mm]
  \bottomrule
\end{tabular}

==> tables/casestudy-vuldee-2-LRP.tex <==
\begin{codelst}
(*@\hlc[con!2]{int}@*) (*@\hlc[con!69]{FUN0}@*) (*@\hlc[pro!4]{(}@*) (*@\hlc[pro!37]{int}@*) (*@\hlc[con!73]{VAR0}@*) (*@\hlc[pro!84]{,}@*) (*@\hlc[pro!30]{char}@*) (*@\hlc[pro!51]{*}@*) (*@\hlc[pro!16]{VAR1}@*) (*@\hlc[con!6]{[}@*) (*@\hlc[pro!13]{]}@*) (*@\hlc[pro!4]{)}@*)
(*@\hlc[pro!38]{VAR0}@*) (*@\hlc[pro!3]{=}@*) (*@\hlc[con!38]{malloc}@*) (*@\hlc[con!2]{(}@*) (*@\hlc[con!1]{INT0}@*) (*@\hlc[con!2]{)}@*) (*@\hlc[pro!15]{;}@*)
(*@\hlc[con!100]{strcpy}@*) (*@\hlc[con!4]{(}@*) (*@\hlc[pro!35]{VAR0}@*) (*@\hlc[con!7]{,}@*) (*@\hlc[pro!10]{VAR1}@*) (*@\hlc[con!7]{[}@*) (*@\hlc[con!20]{INT0}@*) (*@\hlc[pro!3]{]}@*) (*@\hlc[con!1]{)}@*) (*@\hlc[pro!14]{;}@*)
\end{codelst}

==> tables/casestudy-vuldee-2-Lemna.tex <==
\begin{codelst}
(*@\hlc[con!64]{int}@*) (*@\hlc[con!15]{FUN0}@*) (*@\hlc[con!13]{(}@*) (*@\hlc[con!13]{int}@*) (*@\hlc[con!13]{VAR0}@*) (*@\hlc[pro!8]{,}@*) (*@\hlc[pro!8]{char}@*) (*@\hlc[pro!8]{*}@*) (*@\hlc[pro!16]{VAR1}@*) (*@\hlc[pro!16]{[}@*) (*@\hlc[pro!27]{]}@*) (*@\hlc[pro!27]{)}@*)
(*@\hlc[pro!27]{VAR0}@*) (*@\hlc[pro!27]{=}@*) (*@\hlc[pro!59]{malloc}@*) (*@\hlc[con!11]{(}@*) (*@\hlc[con!93]{INT0}@*) (*@\hlc[con!73]{)}@*) (*@\hlc[pro!75]{;}@*)
(*@\hlc[pro!77]{strcpy}@*) (*@\hlc[pro!77]{(}@*) (*@\hlc[pro!77]{VAR0}@*) (*@\hlc[pro!77]{,}@*) (*@\hlc[pro!100]{VAR1}@*) (*@\hlc[pro!14]{[}@*) (*@\hlc[pro!14]{INT0}@*) (*@\hlc[pro!14]{]}@*) (*@\hlc[pro!14]{)}@*) (*@\hlc[pro!35]{;}@*)
\end{codelst}

==> tables/casestudy-vuldee-lemna.tex <==
\begin{codelst}
(*@\hlc[pro!31]{INT0}@*) (*@\hlc[pro!31]{]}@*) (*@\hlc[pro!31]{;}@*)
(*@\hlc[pro!31]{VAR0}@*) (*@\hlc[pro!31]{[}@*) (*@\hlc[pro!32]{INT0}@*) (*@\hlc[pro!33]{]}@*) (*@\hlc[pro!33]{=}@*) (*@\hlc[pro!34]{STR0}@*) (*@\hlc[pro!35]{;}@*)
(*@\hlc[pro!36]{wchar\_t}@*) (*@\hlc[pro!37]{VAR0}@*) (*@\hlc[pro!39]{[}@*) (*@\hlc[pro!40]{INT0}@*) (*@\hlc[pro!41]{]}@*) (*@\hlc[pro!43]{;}@*)
(*@\hlc[pro!45]{wmemset}@*) (*@\hlc[pro!62]{(}@*) (*@\hlc[pro!64]{VAR0}@*) (*@\hlc[pro!66]{,}@*) (*@\hlc[pro!68]{STR0}@*) (*@\hlc[pro!69]{,}@*) (*@\hlc[pro!71]{INT0}@*) (*@\hlc[pro!97]{-}@*) (*@\hlc[pro!98]{INT1}@*) (*@\hlc[pro!99]{)}@*) (*@\hlc[pro!100]{;}@*)
(*@\hlc[pro!100]{VAR0}@*) (*@\hlc[pro!100]{[}@*) (*@\hlc[pro!99]{INT0}@*) (*@\hlc[pro!98]{-}@*) (*@\hlc[pro!97]{INT1}@*) (*@\hlc[pro!43]{]}@*) (*@\hlc[pro!41]{=}@*) (*@\hlc[pro!39]{STR0}@*) (*@\hlc[pro!37]{;}@*)
(*@\hlc[pro!36]{memmove}@*) (*@\hlc[pro!34]{(}@*) (*@\hlc[pro!32]{VAR0}@*) (*@\hlc[pro!30]{,}@*) (*@\hlc[pro!29]{VAR1}@*) (*@\hlc[pro!27]{,}@*) (*@\hlc[pro!26]{INT0}@*) (*@\hlc[pro!24]{*}@*) (*@\hlc[pro!23]{sizeof}@*) (*@\hlc[pro!22]{(}@*) (*@\hlc[pro!21]{wchar\_t}@*) (*@\hlc[pro!21]{)}@*) (*@\hlc[pro!20]{)}@*) (*@\hlc[pro!20]{;}@*)
\end{codelst}

==> tables/casestudy-vuldee-lrp.tex <==
\begin{codelst}
(*@\hlc[pro!18]{INT0}@*) (*@\hlc[con!2]{]}@*) (*@\hlc[con!6]{;}@*)
(*@\hlc[con!10]{VAR0}@*) (*@\hlc[con!1]{[}@*) (*@\hlc[con!23]{INT0}@*) (*@\hlc[pro!13]{]}@*) (*@\hlc[con!21]{=}@*) (*@\hlc[con!21]{STR0}@*) (*@\hlc[con!9]{;}@*)
(*@\hlc[con!1]{wchar\_t}@*) (*@\hlc[con!30]{VAR0}@*) (*@\hlc[con!5]{[}@*) (*@\hlc[pro!100]{INT0}@*) (*@\hlc[pro!43]{]}@*) (*@\hlc[con!19]{;}@*)
(*@\hlc[con!28]{wmemset}@*) (*@\hlc[pro!4]{(}@*) (*@\hlc[con!29]{VAR0}@*) (*@\hlc[pro!12]{,}@*) (*@\hlc[con!7]{STR0}@*) (*@\hlc[pro!12]{,}@*) (*@\hlc[con!1]{INT0}@*) (*@\hlc[pro!22]{-}@*) (*@\hlc[pro!30]{INT1}@*) (*@\hlc[con!10]{)}@*) (*@\hlc[pro!2]{;}@*)
(*@\hlc[pro!3]{VAR0}@*) (*@\hlc[con!7]{[}@*) (*@\hlc[pro!0]{INT0}@*) (*@\hlc[pro!8]{-}@*) (*@\hlc[pro!19]{INT1}@*) (*@\hlc[pro!9]{]}@*) (*@\hlc[pro!2]{=}@*) (*@\hlc[con!35]{STR0}@*) (*@\hlc[con!0]{;}@*)
(*@\hlc[pro!10]{memmove}@*) (*@\hlc[con!5]{(}@*) (*@\hlc[pro!1]{VAR0}@*) (*@\hlc[con!3]{,}@*) (*@\hlc[pro!3]{VAR1}@*) (*@\hlc[con!4]{,}@*) (*@\hlc[con!5]{INT0}@*) (*@\hlc[con!1]{*}@*) (*@\hlc[con!4]{sizeof}@*) (*@\hlc[con!1]{(}@*) (*@\hlc[con!1]{wchar\_t}@*) (*@\hlc[con!2]{)}@*) (*@\hlc[con!2]{)}@*) (*@\hlc[pro!0]{;}@*)
\end{codelst}

==> tables/casestudy_bifold_damd.tex <==
\begin{tabular}{
  cl
}
  \toprule
  \bfseries Id & \bfseries LRP\\
  \midrule
  0 & \cellcolor{pro!7} \ttfamily invoke-virtual \\
  1 & \cellcolor{pro!27} \ttfamily move-result-object \\
  2 & \cellcolor{pro!48} \ttfamily if-eqz \\
  3 & \cellcolor{pro!33} \ttfamily const-string \\
  4 & \cellcolor{pro!28} \ttfamily invoke-virtual \\
  5 & \cellcolor{pro!17} \ttfamily move-result-object \\
  6 & \cellcolor{pro!56} \ttfamily check-cast \\
  7 & \cellcolor{pro!99} \ttfamily array-length \\
  8 & \cellcolor{pro!48} \ttfamily new-array \\
  9 & \cellcolor{pro!13} \ttfamily const/4 \\
  10 & \cellcolor{pro!5} \ttfamily array-length \\
  11 & \cellcolor{pro!14} \ttfamily if-ge \\
  12 & \cellcolor{pro!6} \ttfamily aget-object \\
  \bottomrule
\end{tabular}

==> tables/casestudy_bifold_drebin.tex <==
\begin{tabular}{
  cl
}
  \toprule
  \bfseries Id & \bfseries IG\\
  \midrule
  0 & \cellcolor{pro!100} \ttfamily permission::android.permission.SEND\_SMS \\
  1 & \cellcolor{pro!71} \ttfamily call::getSubscriberId \\
  2 & \cellcolor{pro!69} \ttfamily permission::android.permission.READ\_SMS \\
  3 & \cellcolor{pro!53} \ttfamily permission::android.permission.READ\_PHONE\_STATE \\
  4 & \cellcolor{pro!53} \ttfamily permission::android.permission.INTERNET \\
  5 & \cellcolor{pro!47} \ttfamily feature::android.hardware.telephony \\
  6 & \cellcolor{pro!45} \ttfamily intent::android.intent.action.PHONE\_STATE \\
  7 & \cellcolor{pro!41} \ttfamily permission::android.permission.DELETE\_PACKAGES \\
  8 & \cellcolor{pro!41} \ttfamily call::sendSMS \\
  9 & \cellcolor{pro!39} \ttfamily permission::android.permission.INSTALL\_PACKAGES \\
  10 & \cellcolor{pro!34} \ttfamily provider::android.provider.Telephony.SMS\_RECEIVED \\
  11 & \cellcolor{pro!34} \ttfamily call::getDeviceId \\
  12 & \cellcolor{pro!32} \ttfamily api\_call::android/telephony/TelephonyManager;-\textgreater{}getDeviceId \\
  13 & \cellcolor{pro!32} \ttfamily api\_call::android/content/Context;-\textgreater{}startService \\
  14 & \cellcolor{pro!32} \ttfamily permission::android.permission.WRITE\_EXTERNAL\_STORAGE \\
  15 & \cellcolor{pro!29} \ttfamily url::lebar.gicp.net \\
  16 & \cellcolor{pro!28} \ttfamily activity::.readme \\
  17 & \cellcolor{pro!28} \ttfamily activity::.TingTing21 \\
  18 & \cellcolor{pro!25} \ttfamily intent::android.intent.action.BOOT\_COMPLETED \\
  19 & \cellcolor{pro!19} \ttfamily permission::android.permission.RECEIVE\_SMS \\
  20 & \cellcolor{pro!16} \ttfamily permission::android.permission.ACCESS\_WIFI\_STATE \\
  21 & \cellcolor{pro!12} \ttfamily intent::android.intent.action.MAIN \\
  22 & \cellcolor{pro!12} \ttfamily service\_receiver::Market \\
  23 & \cellcolor{pro!12} \ttfamily intent::android.intent.action.NEW\_OUTGOING\_CALL \\
  24 & \cellcolor{pro!11} \ttfamily feature::android.hardware.location.network \\
  25 & \cellcolor{pro!10} \ttfamily url::www.gstatic.com \\
  26 & \cellcolor{pro!9} \ttfamily permission::android.permission.RECEIVE\_BOOT\_COMPLETED \\
  27 & \cellcolor{pro!6} \ttfamily service\_receiver::com.GoldDream.zj.zjReceiver \\
  28 & \cellcolor{pro!4} \ttfamily call::getPackageInfo \\
  29 & \cellcolor{pro!3} \ttfamily feature::android.hardware.wifi \\
  30 & \cellcolor{pro!3} \ttfamily url::http://lebar.gicp.net/more.aspx?pid\%3D9963\&cid\%3D1000 \\
  31 & \cellcolor{pro!2} \ttfamily url::http://schemas.android.com/apk/lib/com.google.ads \\
  32 & \cellcolor{pro!2} \ttfamily call::Cipher(AES/CBC/PKCS5Padding) \\
  33 & \cellcolor{con!0} \ttfamily url::http://www.gstatic.com/afma/sdk-core-v40.js\textbackslash{} \\
  34 & \cellcolor{con!1} \ttfamily url::http://lebar.gicp.net/update\_soft.aspx?pid\%3D9963\&cid\%3D1000 \\
  35 & \cellcolor{con!2} \ttfamily permission::android.permission.PROCESS\_OUTGOING\_CALLS \\
  36 & \cellcolor{con!3} \ttfamily real\_permission::android.permission.ACCESS\_NETWORK\_STATE \\
  37 & \cellcolor{con!3} \ttfamily call::printStackTrace \\
  38 & \cellcolor{con!4} \ttfamily feature::android.hardware.location.gps \\
  39 & \cellcolor{con!7} \ttfamily api\_call::android/webkit/WebView \\
  40 & \cellcolor{con!8} \ttfamily real\_permission::android.permission.SEND\_SMS \\
  41 & \cellcolor{con!9} \ttfamily api\_call::android/telephony/SmsManager;-\textgreater{}sendTextMessage \\
  42 & \cellcolor{con!11} \ttfamily url::a.admob.com \\
  43 & \cellcolor{con!11} \ttfamily feature::android.hardware.location \\
  44 & \cellcolor{con!12} \ttfamily permission::android.permission.ACCESS\_COARSE\_LOCATION \\
  45 & \cellcolor{con!13} \ttfamily url::http://a.admob.com/f0? \\
  46 & \cellcolor{con!19} \ttfamily permission::android.permission.ACCESS\_NETWORK\_STATE \\
  47 & \cellcolor{con!25} \ttfamily api\_call::android/net/ConnectivityManager;-\textgreater{}getActiveNetworkInfo \\
  48 & \cellcolor{con!25} \ttfamily permission::android.permission.ACCESS\_FINE\_LOCATION \\
  49 & \cellcolor{con!27} \ttfamily real\_permission::android.permission.READ\_PHONE\_STATE \\
  50 & \cellcolor{con!35} \ttfamily call::getSystemService \\
  51 & \cellcolor{con!37} \ttfamily url::schemas.android.com \\
  52 & \cellcolor{con!39} \ttfamily real\_permission::android.permission.INTERNET \\
  53 & \cellcolor{con!50} \ttfamily permission::android.permission.CALL\_PHONE \\
  54 & \cellcolor{con!55} \ttfamily feature::android.hardware.touchscreen \\
  55 & \cellcolor{con!60} \ttfamily intent::android.intent.category.LAUNCHER \\
  \bottomrule
\end{tabular}

==> tables/intro-igLong.tex <==
\begin{codelst}
(*@\hlc[pro!16]{VAR0}@*) (*@\hlc[pro!8]{=}@*) (*@\hlc[pro!40]{FUN0}@*) (*@\hlc[pro!10]{(}@*) (*@\hlc[pro!22]{VAR1}@*) (*@\hlc[con!7]{[}@*) (*@\hlc[pro!16]{VAR2}@*) (*@\hlc[con!32]{]}@*) (*@\hlc[pro!30]{,}@*) (*@\hlc[pro!57]{STR0}@*) (*@\hlc[pro!31]{,}@*) (*@\hlc[pro!100]{\&}@*) (*@\hlc[pro!26]{VAR3}@*) (*@\hlc[con!3]{)}@*) (*@\hlc[pro!1]{;}@*)
(*@\hlc[con!17]{VAR0}@*) (*@\hlc[pro!15]{=}@*) (*@\hlc[pro!46]{strcpy}@*) (*@\hlc[con!1]{(}@*) (*@\hlc[pro!12]{(}@*) (*@\hlc[pro!69]{FUN0}@*) (*@\hlc[con!5]{(}@*) (*@\hlc[pro!86]{strlen}@*) (*@\hlc[pro!15]{(}@*) (*@\hlc[pro!30]{VAR1}@*) (*@\hlc[pro!70]{[}@*) (*@\hlc[pro!56]{INT0}@*) (*@\hlc[pro!35]{]}@*) (*@\hlc[pro!19]{)}@*) (*@\hlc[pro!88]{+}@*) (*@\hlc[pro!64]{INT0}@*) (*@\hlc[pro!30]{)}@*) (*@\hlc[pro!29]{)}@*) (*@\hlc[pro!53]{,}@*) (*@\hlc[pro!49]{VAR1}@*) (*@\hlc[pro!61]{[}@*) (*@\hlc[pro!33]{INT0}@*) (*@\hlc[con!51]{]}@*) (*@\hlc[pro!56]{)}@*) (*@\hlc[con!44]{;}@*)
\end{codelst}

==> tables/vamos.tex <==
\begin{tabular}{
  cll
}
  \toprule
  \bfseries Id & \bfseries LRP\\
  \midrule
  0 & \cellcolor{pro!2} \ttfamily gfn_mod_map \\\\[ -3.2mm]
  1 & \cellcolor{pro!2} \ttfamily gfn_file_open \\\\[ -3.2mm]
  2 & \cellcolor{pro!23} \ttfamily gfn_sck_create \\\\[ -3.2mm]
  3 & \cellcolor{pro!15} \ttfamily gfn_sck_bind \\\\[ -3.2mm]
  4 & \cellcolor{pro!100} \ttfamily gfn_sck_listen \\\\[ -3.2mm]
  5 & \cellcolor{pro!28} \ttfamily gfn_sck_create \\\\[ -3.2mm]
  6 & \cellcolor{pro!8} \ttfamily gfn_sck_accept \\\\[ -3.2mm]
  7 & \cellcolor{pro!0} \ttfamily ... \\\\[ -3.2mm]
  7 & \cellcolor{con!2} \ttfamily gfn_mod_get_handle \\\\[ -3.2mm]
  7 & \cellcolor{pro!5} \ttfamily gfn_mem_free \\\\[ -3.2mm]
  7 & \cellcolor{pro!10} \ttfamily gfn_sck_create \\\\[ -3.2mm]
  8 & \cellcolor{pro!30} \ttfamily gfn_sck_bind \\\\[ -3.2mm]
  8 & \cellcolor{pro!62} \ttfamily gfn_sck_recv \\\\[ -3.2mm]
  8 & \cellcolor{con!1} \ttfamily gfn_sck_send \\\\[ -3.2mm]
  8 & \cellcolor{pro!0} \ttfamily gfn_proc_get_info \\\\[ -3.2mm]
  \bottomrule
\end{tabular}
